Adaptive Neural Signal Detection for Massive MIMO

Symbol detection for Massive Multiple-Input Multiple-Output (MIMO) is a challenging problem for which traditional algorithms are either impractical or suffer from performance limitations. Several recently proposed learning-based approaches achieve promising results on simple channel models (e.g., i.i.d. Gaussian). However, their performance degrades significantly on real-world channels with spatial correlation. We propose MMNet, a deep learning MIMO detection scheme that significantly outperforms existing approaches on realistic channels with the same or lower computational complexity. MMNet's design builds on the theory of iterative soft-thresholding algorithms and uses a novel training algorithm that leverages temporal and spectral correlation to accelerate training. Together, these innovations allow MMNet to train online for every realization of the channel. On i.i.d. Gaussian channels, MMNet requires two orders of magnitude fewer operations than existing deep learning schemes but achieves near-optimal performance. On spatially-correlated channels, it achieves the same error rate as the next-best learning scheme (OAMPNet) at 2.5dB lower SNR and with at least 10x less computational complexity. MMNet is also 4--8dB better overall than a classic linear scheme like the minimum mean square error (MMSE) detector.

==> correlated.tex <==
\chapter{Correlated Channels}\label{ch:correlated}
In this chapter, we will first discuss why considering \gls{iid} channels is not sufficient in practice. We then explain the simulator we used to generate the real channel samples. The \sys proposal for the correlated channels and its error dynamics follows next. We will finish this chapter by discussing the solutions to even further reduce the cost of \sys in practical schemes.   
\section{What happens in correlated channels?}
\Cref{fig:H00} shows the SER-SNR curve for a channel realization from our simulator discussed in \cref{sec:sim} for which an astonishing $\approx$11dB performance difference between MMSE and ML at SER of 0.01 is obtained. This deviation can be huge comparing with 2-3dB difference we used to have for iid channels in \Cref{ch:iid}. As we see in~\Cref{fig:H00}, even OAMPNet which has shown promising performance improvements relative to OAMP under a very simple correlation model in \cite{he2018model}, will drastically withdraw in accuracy in a realistic channel scenario. In this section, we will propose \sys for more realistic channel correlation.
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/setup.png}
%     \caption{Setup. }
%     \label{fig:my_label}
% \end{figure}


% Regarding the two terms in error dynamic equation \ref{eq:err_dynamics}, basically there are two thing important for us. First, we want to decrease the power of noise and second, we want to avoid building up error correlations among different transmitters detected symbols. This means having almost diagonal diagonal auto-covariance matrices with traces moving to zero.

\begin{align*}
    \textbf{z}_t &= \xh_{t} + \boldsymbol{\Theta}_t^{(1)} (\y - \Hb\xh_t)\\
\end{align*}





==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_learnW_0.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 1.000000)
(17.552568, 1.000000)
(18.638512, 1.000000)
(18.546717, 1.000000)
(13.428638, 1.000000)
(16.794140, 1.000000)
(14.297143, 1.000000)
(17.171722, 0.937500)
(20.059292, 1.000000)
(11.256145, 1.000000)
(25.958267, 1.000000)
(14.636854, 1.000000)
(16.587755, 1.000000)
(8.500388, 1.000000)
(19.118383, 1.000000)
(19.355614, 1.000000)
(16.919485, 1.000000)
(10.740816, 1.000000)
(24.433674, 1.000000)
(15.328254, 1.000000)
(15.667542, 1.000000)
(32.651962, 1.000000)
(14.833853, 1.000000)
(24.772644, 1.000000)
(19.206205, 1.000000)
(18.807907, 1.000000)
(20.472019, 1.000000)
(24.486319, 1.000000)
(13.134361, 1.000000)
(14.394195, 1.000000)
(16.070848, 1.000000)
(25.167027, 1.000000)
(15.581610, 1.000000)
(17.096106, 1.000000)
(21.280998, 1.000000)
(23.876585, 1.000000)
(13.036207, 1.000000)
(22.731215, 1.000000)
(35.325077, 1.000000)
(24.573538, 1.000000)
(22.238827, 1.000000)
(17.241997, 1.000000)
(21.504358, 1.000000)
(16.334728, 1.000000)
(18.660828, 1.000000)
(10.326597, 1.000000)
(16.468248, 1.000000)
(13.946894, 1.000000)
(33.479321, 1.000000)
(13.391328, 1.000000)
(16.313137, 1.000000)
(17.417023, 1.000000)
(14.955702, 1.000000)
(23.593338, 1.000000)
(25.343109, 1.000000)
(28.576508, 1.000000)
(26.743855, 1.000000)
(17.670483, 1.000000)
(14.859500, 1.000000)
(13.146446, 1.000000)
(16.851610, 1.000000)
(24.674076, 1.000000)
(14.513160, 1.000000)
(18.443485, 1.000000)
(13.139583, 1.000000)
(13.289401, 1.000000)
(13.496741, 1.000000)
(17.107384, 1.000000)
(9.916093, 1.000000)
(12.541000, 0.968750)
(13.952982, 1.000000)
(19.874964, 1.000000)
(36.316109, 1.000000)
(14.172893, 1.000000)
(8.225883, 1.000000)
(13.984437, 1.000000)
(32.250385, 1.000000)
(20.073103, 1.000000)
(18.860682, 1.000000)
(21.450701, 1.000000)
(12.890105, 1.000000)
(20.801798, 1.000000)
(20.644512, 0.968750)
(19.323544, 1.000000)
(12.121391, 1.000000)
(15.076665, 1.000000)
(15.545311, 1.000000)
(15.126464, 1.000000)
(8.966540, 1.000000)
(14.076862, 1.000000)
(18.888176, 1.000000)
(12.218390, 1.000000)
(27.091944, 1.000000)
(8.184272, 1.000000)
(21.078032, 0.937500)
(34.766178, 1.000000)
(24.455320, 1.000000)
(9.089629, 1.000000)
(18.335535, 1.000000)
(10.185403, 1.000000)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_learnW_1.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 0.750000)
(17.552568, 0.906250)
(18.638512, 1.000000)
(18.546717, 0.968750)
(13.428638, 0.875000)
(16.794140, 0.687500)
(14.297143, 1.000000)
(17.171722, 0.937500)
(20.059292, 0.812500)
(11.256145, 0.906250)
(25.958267, 0.906250)
(14.636854, 0.687500)
(16.587755, 1.000000)
(8.500388, 0.875000)
(19.118383, 0.875000)
(19.355614, 0.718750)
(16.919485, 0.968750)
(10.740816, 0.750000)
(24.433674, 1.000000)
(15.328254, 0.812500)
(15.667542, 0.906250)
(32.651962, 0.750000)
(14.833853, 1.000000)
(24.772644, 0.937500)
(19.206205, 0.781250)
(18.807907, 0.687500)
(20.472019, 0.812500)
(24.486319, 0.937500)
(13.134361, 0.812500)
(14.394195, 0.937500)
(16.070848, 0.781250)
(25.167027, 0.781250)
(15.581610, 0.625000)
(17.096106, 0.750000)
(21.280998, 0.968750)
(23.876585, 0.937500)
(13.036207, 0.937500)
(22.731215, 0.875000)
(35.325077, 0.937500)
(24.573538, 0.937500)
(22.238827, 0.656250)
(17.241997, 0.781250)
(21.504358, 1.000000)
(16.334728, 0.687500)
(18.660828, 0.718750)
(10.326597, 0.906250)
(16.468248, 0.687500)
(13.946894, 0.906250)
(33.479321, 1.000000)
(13.391328, 0.781250)
(16.313137, 0.656250)
(17.417023, 0.750000)
(14.955702, 0.531250)
(23.593338, 0.812500)
(25.343109, 0.781250)
(28.576508, 0.843750)
(26.743855, 0.906250)
(17.670483, 0.937500)
(14.859500, 0.750000)
(13.146446, 0.906250)
(16.851610, 0.875000)
(24.674076, 0.906250)
(14.513160, 0.750000)
(18.443485, 0.656250)
(13.139583, 0.718750)
(13.289401, 0.781250)
(13.496741, 0.937500)
(17.107384, 1.000000)
(9.916093, 0.906250)
(12.541000, 0.937500)
(13.952982, 0.843750)
(19.874964, 0.718750)
(36.316109, 1.000000)
(14.172893, 0.843750)
(8.225883, 0.781250)
(13.984437, 0.687500)
(32.250385, 0.937500)
(20.073103, 0.937500)
(18.860682, 0.781250)
(21.450701, 0.687500)
(12.890105, 1.000000)
(20.801798, 0.656250)
(20.644512, 0.937500)
(19.323544, 0.625000)
(12.121391, 0.937500)
(15.076665, 0.843750)
(15.545311, 0.687500)
(15.126464, 0.812500)
(8.966540, 0.875000)
(14.076862, 0.687500)
(18.888176, 0.656250)
(12.218390, 0.750000)
(27.091944, 0.781250)
(8.184272, 0.875000)
(21.078032, 0.781250)
(34.766178, 1.000000)
(24.455320, 0.968750)
(9.089629, 0.656250)
(18.335535, 0.718750)
(10.185403, 0.718750)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_learnW_2.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 1.000000)
(17.552568, 1.000000)
(18.638512, 1.000000)
(18.546717, 1.000000)
(13.428638, 1.000000)
(16.794140, 0.500000)
(14.297143, 1.000000)
(17.171722, 0.937500)
(20.059292, 0.562500)
(11.256145, 1.000000)
(25.958267, 0.750000)
(14.636854, 0.812500)
(16.587755, 1.000000)
(8.500388, 1.000000)
(19.118383, 0.875000)
(19.355614, 0.625000)
(16.919485, 1.000000)
(10.740816, 1.000000)
(24.433674, 0.875000)
(15.328254, 0.718750)
(15.667542, 1.000000)
(32.651962, 0.343750)
(14.833853, 1.000000)
(24.772644, 0.750000)
(19.206205, 0.812500)
(18.807907, 0.843750)
(20.472019, 0.875000)
(24.486319, 0.500000)
(13.134361, 0.968750)
(14.394195, 1.000000)
(16.070848, 0.968750)
(25.167027, 0.750000)
(15.581610, 1.000000)
(17.096106, 0.906250)
(21.280998, 0.968750)
(23.876585, 0.718750)
(13.036207, 1.000000)
(22.731215, 0.750000)
(35.325077, 0.625000)
(24.573538, 0.750000)
(22.238827, 0.625000)
(17.241997, 0.906250)
(21.504358, 0.843750)
(16.334728, 0.937500)
(18.660828, 0.875000)
(10.326597, 1.000000)
(16.468248, 0.781250)
(13.946894, 1.000000)
(33.479321, 0.593750)
(13.391328, 0.937500)
(16.313137, 0.906250)
(17.417023, 1.000000)
(14.955702, 0.812500)
(23.593338, 0.750000)
(25.343109, 0.625000)
(28.576508, 0.562500)
(26.743855, 0.625000)
(17.670483, 1.000000)
(14.859500, 0.906250)
(13.146446, 0.937500)
(16.851610, 0.875000)
(24.674076, 0.593750)
(14.513160, 0.968750)
(18.443485, 0.906250)
(13.139583, 0.968750)
(13.289401, 1.000000)
(13.496741, 1.000000)
(17.107384, 1.000000)
(9.916093, 1.000000)
(12.541000, 1.000000)
(13.952982, 1.000000)
(19.874964, 0.656250)
(36.316109, 0.562500)
(14.172893, 1.000000)
(8.225883, 1.000000)
(13.984437, 0.937500)
(32.250385, 0.625000)
(20.073103, 0.875000)
(18.860682, 0.750000)
(21.450701, 1.000000)
(12.890105, 0.968750)
(20.801798, 0.812500)
(20.644512, 0.875000)
(19.323544, 0.312500)
(12.121391, 1.000000)
(15.076665, 0.937500)
(15.545311, 0.593750)
(15.126464, 0.656250)
(8.966540, 1.000000)
(14.076862, 0.750000)
(18.888176, 0.593750)
(12.218390, 1.000000)
(27.091944, 0.406250)
(8.184272, 1.000000)
(21.078032, 0.812500)
(34.766178, 0.625000)
(24.455320, 0.781250)
(9.089629, 0.968750)
(18.335535, 0.812500)
(10.185403, 1.000000)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_learnW_3.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 1.000000)
(17.552568, 1.000000)
(18.638512, 1.000000)
(18.546717, 1.000000)
(13.428638, 1.000000)
(16.794140, 0.625000)
(14.297143, 1.000000)
(17.171722, 1.000000)
(20.059292, 0.750000)
(11.256145, 1.000000)
(25.958267, 0.781250)
(14.636854, 0.968750)
(16.587755, 1.000000)
(8.500388, 1.000000)
(19.118383, 0.937500)
(19.355614, 0.687500)
(16.919485, 1.000000)
(10.740816, 1.000000)
(24.433674, 0.843750)
(15.328254, 1.000000)
(15.667542, 1.000000)
(32.651962, 0.531250)
(14.833853, 1.000000)
(24.772644, 0.843750)
(19.206205, 0.968750)
(18.807907, 0.937500)
(20.472019, 1.000000)
(24.486319, 0.500000)
(13.134361, 1.000000)
(14.394195, 1.000000)
(16.070848, 1.000000)
(25.167027, 0.781250)
(15.581610, 1.000000)
(17.096106, 0.906250)
(21.280998, 1.000000)
(23.876585, 0.812500)
(13.036207, 1.000000)
(22.731215, 0.750000)
(35.325077, 0.437500)
(24.573538, 0.906250)
(22.238827, 0.781250)
(17.241997, 1.000000)
(21.504358, 0.875000)
(16.334728, 1.000000)
(18.660828, 1.000000)
(10.326597, 1.000000)
(16.468248, 1.000000)
(13.946894, 1.000000)
(33.479321, 0.593750)
(13.391328, 1.000000)
(16.313137, 1.000000)
(17.417023, 1.000000)
(14.955702, 0.968750)
(23.593338, 0.843750)
(25.343109, 0.531250)
(28.576508, 0.718750)
(26.743855, 0.687500)
(17.670483, 1.000000)
(14.859500, 0.937500)
(13.146446, 0.968750)
(16.851610, 1.000000)
(24.674076, 0.593750)
(14.513160, 1.000000)
(18.443485, 1.000000)
(13.139583, 1.000000)
(13.289401, 1.000000)
(13.496741, 1.000000)
(17.107384, 1.000000)
(9.916093, 1.000000)
(12.541000, 1.000000)
(13.952982, 1.000000)
(19.874964, 0.843750)
(36.316109, 0.281250)
(14.172893, 1.000000)
(8.225883, 1.000000)
(13.984437, 1.000000)
(32.250385, 0.531250)
(20.073103, 0.906250)
(18.860682, 0.875000)
(21.450701, 1.000000)
(12.890105, 1.000000)
(20.801798, 0.875000)
(20.644512, 0.968750)
(19.323544, 0.562500)
(12.121391, 1.000000)
(15.076665, 1.000000)
(15.545311, 0.781250)
(15.126464, 0.812500)
(8.966540, 1.000000)
(14.076862, 0.875000)
(18.888176, 0.750000)
(12.218390, 1.000000)
(27.091944, 0.531250)
(8.184272, 1.000000)
(21.078032, 0.937500)
(34.766178, 0.656250)
(24.455320, 0.937500)
(9.089629, 1.000000)
(18.335535, 0.906250)
(10.185403, 1.000000)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_learnW_5.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 1.000000)
(17.552568, 1.000000)
(18.638512, 1.000000)
(18.546717, 1.000000)
(13.428638, 1.000000)
(16.794140, 0.750000)
(14.297143, 1.000000)
(17.171722, 1.000000)
(20.059292, 0.750000)
(11.256145, 1.000000)
(25.958267, 0.937500)
(14.636854, 1.000000)
(16.587755, 1.000000)
(8.500388, 1.000000)
(19.118383, 1.000000)
(19.355614, 0.656250)
(16.919485, 1.000000)
(10.740816, 1.000000)
(24.433674, 1.000000)
(15.328254, 1.000000)
(15.667542, 1.000000)
(32.651962, 0.718750)
(14.833853, 1.000000)
(24.772644, 1.000000)
(19.206205, 1.000000)
(18.807907, 1.000000)
(20.472019, 1.000000)
(24.486319, 0.781250)
(13.134361, 1.000000)
(14.394195, 1.000000)
(16.070848, 1.000000)
(25.167027, 0.875000)
(15.581610, 1.000000)
(17.096106, 1.000000)
(21.280998, 1.000000)
(23.876585, 1.000000)
(13.036207, 1.000000)
(22.731215, 0.875000)
(35.325077, 0.750000)
(24.573538, 1.000000)
(22.238827, 0.968750)
(17.241997, 1.000000)
(21.504358, 0.968750)
(16.334728, 1.000000)
(18.660828, 1.000000)
(10.326597, 1.000000)
(16.468248, 1.000000)
(13.946894, 1.000000)
(33.479321, 0.687500)
(13.391328, 1.000000)
(16.313137, 1.000000)
(17.417023, 1.000000)
(14.955702, 1.000000)
(23.593338, 0.937500)
(25.343109, 0.625000)
(28.576508, 0.937500)
(26.743855, 0.750000)
(17.670483, 1.000000)
(14.859500, 1.000000)
(13.146446, 0.968750)
(16.851610, 1.000000)
(24.674076, 0.781250)
(14.513160, 1.000000)
(18.443485, 1.000000)
(13.139583, 1.000000)
(13.289401, 1.000000)
(13.496741, 1.000000)
(17.107384, 1.000000)
(9.916093, 1.000000)
(12.541000, 1.000000)
(13.952982, 1.000000)
(19.874964, 0.843750)
(36.316109, 0.281250)
(14.172893, 1.000000)
(8.225883, 1.000000)
(13.984437, 1.000000)
(32.250385, 0.656250)
(20.073103, 1.000000)
(18.860682, 0.968750)
(21.450701, 1.000000)
(12.890105, 1.000000)
(20.801798, 0.906250)
(20.644512, 0.968750)
(19.323544, 0.906250)
(12.121391, 1.000000)
(15.076665, 1.000000)
(15.545311, 1.000000)
(15.126464, 1.000000)
(8.966540, 1.000000)
(14.076862, 0.937500)
(18.888176, 0.843750)
(12.218390, 1.000000)
(27.091944, 0.593750)
(8.184272, 1.000000)
(21.078032, 1.000000)
(34.766178, 0.750000)
(24.455320, 1.000000)
(9.089629, 1.000000)
(18.335535, 1.000000)
(10.185403, 1.000000)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_learnW_6.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 1.000000)
(17.552568, 1.000000)
(18.638512, 1.000000)
(18.546717, 1.000000)
(13.428638, 1.000000)
(16.794140, 0.781250)
(14.297143, 1.000000)
(17.171722, 1.000000)
(20.059292, 0.750000)
(11.256145, 1.000000)
(25.958267, 0.937500)
(14.636854, 1.000000)
(16.587755, 1.000000)
(8.500388, 1.000000)
(19.118383, 1.000000)
(19.355614, 0.937500)
(16.919485, 1.000000)
(10.740816, 1.000000)
(24.433674, 1.000000)
(15.328254, 1.000000)
(15.667542, 1.000000)
(32.651962, 0.750000)
(14.833853, 1.000000)
(24.772644, 1.000000)
(19.206205, 1.000000)
(18.807907, 1.000000)
(20.472019, 1.000000)
(24.486319, 0.781250)
(13.134361, 1.000000)
(14.394195, 1.000000)
(16.070848, 1.000000)
(25.167027, 1.000000)
(15.581610, 1.000000)
(17.096106, 1.000000)
(21.280998, 1.000000)
(23.876585, 1.000000)
(13.036207, 1.000000)
(22.731215, 0.875000)
(35.325077, 0.687500)
(24.573538, 1.000000)
(22.238827, 0.968750)
(17.241997, 1.000000)
(21.504358, 0.968750)
(16.334728, 1.000000)
(18.660828, 1.000000)
(10.326597, 1.000000)
(16.468248, 1.000000)
(13.946894, 1.000000)
(33.479321, 0.718750)
(13.391328, 1.000000)
(16.313137, 1.000000)
(17.417023, 1.000000)
(14.955702, 1.000000)
(23.593338, 0.968750)
(25.343109, 0.687500)
(28.576508, 0.906250)
(26.743855, 0.687500)
(17.670483, 1.000000)
(14.859500, 1.000000)
(13.146446, 1.000000)
(16.851610, 1.000000)
(24.674076, 0.843750)
(14.513160, 1.000000)
(18.443485, 1.000000)
(13.139583, 1.000000)
(13.289401, 1.000000)
(13.496741, 1.000000)
(17.107384, 1.000000)
(9.916093, 1.000000)
(12.541000, 1.000000)
(13.952982, 1.000000)
(19.874964, 0.875000)
(36.316109, 0.312500)
(14.172893, 1.000000)
(8.225883, 1.000000)
(13.984437, 1.000000)
(32.250385, 0.687500)
(20.073103, 1.000000)
(18.860682, 1.000000)
(21.450701, 1.000000)
(12.890105, 1.000000)
(20.801798, 0.937500)
(20.644512, 0.968750)
(19.323544, 0.937500)
(12.121391, 1.000000)
(15.076665, 1.000000)
(15.545311, 1.000000)
(15.126464, 1.000000)
(8.966540, 1.000000)
(14.076862, 0.906250)
(18.888176, 0.937500)
(12.218390, 1.000000)
(27.091944, 0.468750)
(8.184272, 1.000000)
(21.078032, 1.000000)
(34.766178, 0.781250)
(24.455320, 1.000000)
(9.089629, 1.000000)
(18.335535, 1.000000)
(10.185403, 1.000000)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_learnW_7.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 1.000000)
(17.552568, 1.000000)
(18.638512, 1.000000)
(18.546717, 1.000000)
(13.428638, 1.000000)
(16.794140, 0.812500)
(14.297143, 1.000000)
(17.171722, 1.000000)
(20.059292, 0.843750)
(11.256145, 1.000000)
(25.958267, 0.937500)
(14.636854, 1.000000)
(16.587755, 1.000000)
(8.500388, 1.000000)
(19.118383, 1.000000)
(19.355614, 0.968750)
(16.919485, 1.000000)
(10.740816, 1.000000)
(24.433674, 1.000000)
(15.328254, 1.000000)
(15.667542, 1.000000)
(32.651962, 0.750000)
(14.833853, 1.000000)
(24.772644, 1.000000)
(19.206205, 1.000000)
(18.807907, 1.000000)
(20.472019, 1.000000)
(24.486319, 0.906250)
(13.134361, 1.000000)
(14.394195, 1.000000)
(16.070848, 1.000000)
(25.167027, 1.000000)
(15.581610, 1.000000)
(17.096106, 1.000000)
(21.280998, 1.000000)
(23.876585, 1.000000)
(13.036207, 1.000000)
(22.731215, 0.906250)
(35.325077, 0.781250)
(24.573538, 1.000000)
(22.238827, 1.000000)
(17.241997, 1.000000)
(21.504358, 1.000000)
(16.334728, 1.000000)
(18.660828, 1.000000)
(10.326597, 1.000000)
(16.468248, 1.000000)
(13.946894, 1.000000)
(33.479321, 0.781250)
(13.391328, 1.000000)
(16.313137, 1.000000)
(17.417023, 1.000000)
(14.955702, 1.000000)
(23.593338, 0.968750)
(25.343109, 0.781250)
(28.576508, 0.968750)
(26.743855, 0.875000)
(17.670483, 1.000000)
(14.859500, 1.000000)
(13.146446, 1.000000)
(16.851610, 1.000000)
(24.674076, 0.843750)
(14.513160, 1.000000)
(18.443485, 1.000000)
(13.139583, 1.000000)
(13.289401, 1.000000)
(13.496741, 1.000000)
(17.107384, 1.000000)
(9.916093, 1.000000)
(12.541000, 1.000000)
(13.952982, 1.000000)
(19.874964, 0.843750)
(36.316109, 0.375000)
(14.172893, 1.000000)
(8.225883, 1.000000)
(13.984437, 1.000000)
(32.250385, 0.750000)
(20.073103, 1.000000)
(18.860682, 0.968750)
(21.450701, 1.000000)
(12.890105, 1.000000)
(20.801798, 0.968750)
(20.644512, 0.968750)
(19.323544, 0.906250)
(12.121391, 1.000000)
(15.076665, 1.000000)
(15.545311, 1.000000)
(15.126464, 1.000000)
(8.966540, 1.000000)
(14.076862, 0.906250)
(18.888176, 1.000000)
(12.218390, 1.000000)
(27.091944, 0.593750)
(8.184272, 1.000000)
(21.078032, 1.000000)
(34.766178, 0.750000)
(24.455320, 1.000000)
(9.089629, 1.000000)
(18.335535, 1.000000)
(10.185403, 1.000000)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_learnW_8.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 1.000000)
(17.552568, 1.000000)
(18.638512, 1.000000)
(18.546717, 1.000000)
(13.428638, 1.000000)
(16.794140, 0.781250)
(14.297143, 1.000000)
(17.171722, 1.000000)
(20.059292, 0.781250)
(11.256145, 1.000000)
(25.958267, 0.906250)
(14.636854, 1.000000)
(16.587755, 1.000000)
(8.500388, 1.000000)
(19.118383, 1.000000)
(19.355614, 1.000000)
(16.919485, 1.000000)
(10.740816, 1.000000)
(24.433674, 1.000000)
(15.328254, 1.000000)
(15.667542, 1.000000)
(32.651962, 0.718750)
(14.833853, 1.000000)
(24.772644, 1.000000)
(19.206205, 1.000000)
(18.807907, 1.000000)
(20.472019, 1.000000)
(24.486319, 0.937500)
(13.134361, 1.000000)
(14.394195, 1.000000)
(16.070848, 1.000000)
(25.167027, 1.000000)
(15.581610, 1.000000)
(17.096106, 1.000000)
(21.280998, 1.000000)
(23.876585, 1.000000)
(13.036207, 1.000000)
(22.731215, 0.937500)
(35.325077, 0.843750)
(24.573538, 1.000000)
(22.238827, 0.968750)
(17.241997, 1.000000)
(21.504358, 1.000000)
(16.334728, 1.000000)
(18.660828, 1.000000)
(10.326597, 1.000000)
(16.468248, 1.000000)
(13.946894, 1.000000)
(33.479321, 0.937500)
(13.391328, 1.000000)
(16.313137, 1.000000)
(17.417023, 1.000000)
(14.955702, 1.000000)
(23.593338, 0.968750)
(25.343109, 0.781250)
(28.576508, 0.968750)
(26.743855, 0.781250)
(17.670483, 1.000000)
(14.859500, 1.000000)
(13.146446, 1.000000)
(16.851610, 1.000000)
(24.674076, 0.843750)
(14.513160, 1.000000)
(18.443485, 1.000000)
(13.139583, 1.000000)
(13.289401, 1.000000)
(13.496741, 1.000000)
(17.107384, 1.000000)
(9.916093, 1.000000)
(12.541000, 1.000000)
(13.952982, 1.000000)
(19.874964, 0.906250)
(36.316109, 0.562500)
(14.172893, 1.000000)
(8.225883, 1.000000)
(13.984437, 1.000000)
(32.250385, 0.843750)
(20.073103, 1.000000)
(18.860682, 1.000000)
(21.450701, 1.000000)
(12.890105, 1.000000)
(20.801798, 0.937500)
(20.644512, 0.968750)
(19.323544, 0.906250)
(12.121391, 1.000000)
(15.076665, 1.000000)
(15.545311, 1.000000)
(15.126464, 1.000000)
(8.966540, 1.000000)
(14.076862, 0.906250)
(18.888176, 1.000000)
(12.218390, 1.000000)
(27.091944, 0.593750)
(8.184272, 1.000000)
(21.078032, 1.000000)
(34.766178, 0.812500)
(24.455320, 1.000000)
(9.089629, 1.000000)
(18.335535, 1.000000)
(10.185403, 1.000000)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_learnW_9.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 1.000000)
(17.552568, 1.000000)
(18.638512, 1.000000)
(18.546717, 1.000000)
(13.428638, 1.000000)
(16.794140, 0.875000)
(14.297143, 1.000000)
(17.171722, 1.000000)
(20.059292, 0.781250)
(11.256145, 1.000000)
(25.958267, 0.937500)
(14.636854, 1.000000)
(16.587755, 1.000000)
(8.500388, 1.000000)
(19.118383, 1.000000)
(19.355614, 1.000000)
(16.919485, 1.000000)
(10.740816, 1.000000)
(24.433674, 1.000000)
(15.328254, 1.000000)
(15.667542, 1.000000)
(32.651962, 0.750000)
(14.833853, 1.000000)
(24.772644, 1.000000)
(19.206205, 1.000000)
(18.807907, 1.000000)
(20.472019, 1.000000)
(24.486319, 0.968750)
(13.134361, 1.000000)
(14.394195, 1.000000)
(16.070848, 1.000000)
(25.167027, 1.000000)
(15.581610, 1.000000)
(17.096106, 1.000000)
(21.280998, 1.000000)
(23.876585, 1.000000)
(13.036207, 1.000000)
(22.731215, 0.937500)
(35.325077, 0.843750)
(24.573538, 1.000000)
(22.238827, 1.000000)
(17.241997, 1.000000)
(21.504358, 1.000000)
(16.334728, 1.000000)
(18.660828, 1.000000)
(10.326597, 1.000000)
(16.468248, 1.000000)
(13.946894, 1.000000)
(33.479321, 0.937500)
(13.391328, 1.000000)
(16.313137, 1.000000)
(17.417023, 1.000000)
(14.955702, 1.000000)
(23.593338, 0.937500)
(25.343109, 0.812500)
(28.576508, 0.937500)
(26.743855, 0.812500)
(17.670483, 1.000000)
(14.859500, 1.000000)
(13.146446, 1.000000)
(16.851610, 1.000000)
(24.674076, 0.937500)
(14.513160, 1.000000)
(18.443485, 1.000000)
(13.139583, 1.000000)
(13.289401, 1.000000)
(13.496741, 1.000000)
(17.107384, 1.000000)
(9.916093, 1.000000)
(12.541000, 1.000000)
(13.952982, 1.000000)
(19.874964, 0.937500)
(36.316109, 0.625000)
(14.172893, 1.000000)
(8.225883, 1.000000)
(13.984437, 1.000000)
(32.250385, 0.750000)
(20.073103, 1.000000)
(18.860682, 1.000000)
(21.450701, 1.000000)
(12.890105, 1.000000)
(20.801798, 0.937500)
(20.644512, 0.968750)
(19.323544, 0.968750)
(12.121391, 1.000000)
(15.076665, 1.000000)
(15.545311, 1.000000)
(15.126464, 1.000000)
(8.966540, 1.000000)
(14.076862, 0.937500)
(18.888176, 1.000000)
(12.218390, 1.000000)
(27.091944, 0.750000)
(8.184272, 1.000000)
(21.078032, 1.000000)
(34.766178, 0.843750)
(24.455320, 1.000000)
(9.089629, 1.000000)
(18.335535, 1.000000)
(10.185403, 1.000000)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_oampW_0.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 1.000000)
(17.552568, 1.000000)
(18.638512, 1.000000)
(18.546717, 1.000000)
(13.428638, 1.000000)
(16.794140, 0.937500)
(14.297143, 1.000000)
(17.171722, 0.906250)
(20.059292, 1.000000)
(11.256145, 1.000000)
(25.958267, 0.937500)
(14.636854, 1.000000)
(16.587755, 1.000000)
(8.500388, 1.000000)
(19.118383, 1.000000)
(19.355614, 1.000000)
(16.919485, 1.000000)
(10.740816, 1.000000)
(24.433674, 1.000000)
(15.328254, 1.000000)
(15.667542, 1.000000)
(32.651962, 1.000000)
(14.833853, 1.000000)
(24.772644, 1.000000)
(19.206205, 1.000000)
(18.807907, 1.000000)
(20.472019, 0.968750)
(24.486319, 1.000000)
(13.134361, 1.000000)
(14.394195, 1.000000)
(16.070848, 1.000000)
(25.167027, 0.937500)
(15.581610, 1.000000)
(17.096106, 1.000000)
(21.280998, 1.000000)
(23.876585, 1.000000)
(13.036207, 1.000000)
(22.731215, 1.000000)
(35.325077, 0.937500)
(24.573538, 0.937500)
(22.238827, 0.937500)
(17.241997, 1.000000)
(21.504358, 1.000000)
(16.334728, 0.937500)
(18.660828, 1.000000)
(10.326597, 1.000000)
(16.468248, 1.000000)
(13.946894, 1.000000)
(33.479321, 0.875000)
(13.391328, 1.000000)
(16.313137, 0.937500)
(17.417023, 1.000000)
(14.955702, 1.000000)
(23.593338, 1.000000)
(25.343109, 1.000000)
(28.576508, 0.906250)
(26.743855, 1.000000)
(17.670483, 0.968750)
(14.859500, 1.000000)
(13.146446, 1.000000)
(16.851610, 1.000000)
(24.674076, 1.000000)
(14.513160, 1.000000)
(18.443485, 1.000000)
(13.139583, 1.000000)
(13.289401, 1.000000)
(13.496741, 0.968750)
(17.107384, 1.000000)
(9.916093, 1.000000)
(12.541000, 1.000000)
(13.952982, 1.000000)
(19.874964, 1.000000)
(36.316109, 0.875000)
(14.172893, 1.000000)
(8.225883, 1.000000)
(13.984437, 1.000000)
(32.250385, 0.937500)
(20.073103, 1.000000)
(18.860682, 1.000000)
(21.450701, 1.000000)
(12.890105, 1.000000)
(20.801798, 1.000000)
(20.644512, 1.000000)
(19.323544, 1.000000)
(12.121391, 1.000000)
(15.076665, 1.000000)
(15.545311, 1.000000)
(15.126464, 1.000000)
(8.966540, 1.000000)
(14.076862, 1.000000)
(18.888176, 0.968750)
(12.218390, 1.000000)
(27.091944, 1.000000)
(8.184272, 1.000000)
(21.078032, 1.000000)
(34.766178, 0.875000)
(24.455320, 0.906250)
(9.089629, 1.000000)
(18.335535, 1.000000)
(10.185403, 1.000000)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_oampW_1.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 0.187500)
(17.552568, 0.312500)
(18.638512, 0.250000)
(18.546717, 0.406250)
(13.428638, 0.093750)
(16.794140, 0.187500)
(14.297143, 0.062500)
(17.171722, 0.187500)
(20.059292, 0.250000)
(11.256145, 0.500000)
(25.958267, 0.375000)
(14.636854, 0.125000)
(16.587755, 0.250000)
(8.500388, 0.500000)
(19.118383, 0.125000)
(19.355614, 0.281250)
(16.919485, 0.062500)
(10.740816, 0.218750)
(24.433674, 0.468750)
(15.328254, 0.187500)
(15.667542, 0.062500)
(32.651962, 0.187500)
(14.833853, 0.000000)
(24.772644, 0.531250)
(19.206205, 0.000000)
(18.807907, 0.031250)
(20.472019, 0.406250)
(24.486319, 0.468750)
(13.134361, 0.125000)
(14.394195, 0.312500)
(16.070848, 0.312500)
(25.167027, 0.281250)
(15.581610, 0.156250)
(17.096106, 0.156250)
(21.280998, 0.531250)
(23.876585, 0.375000)
(13.036207, 0.187500)
(22.731215, 0.093750)
(35.325077, 0.562500)
(24.573538, 0.500000)
(22.238827, 0.187500)
(17.241997, 0.187500)
(21.504358, 0.625000)
(16.334728, 0.062500)
(18.660828, 0.062500)
(10.326597, 0.531250)
(16.468248, 0.031250)
(13.946894, 0.312500)
(33.479321, 0.812500)
(13.391328, 0.156250)
(16.313137, 0.312500)
(17.417023, 0.000000)
(14.955702, 0.031250)
(23.593338, 0.156250)
(25.343109, 0.187500)
(28.576508, 0.406250)
(26.743855, 0.187500)
(17.670483, 0.312500)
(14.859500, 0.093750)
(13.146446, 0.250000)
(16.851610, 0.187500)
(24.674076, 0.156250)
(14.513160, 0.125000)
(18.443485, 0.062500)
(13.139583, 0.000000)
(13.289401, 0.093750)
(13.496741, 0.375000)
(17.107384, 0.062500)
(9.916093, 0.687500)
(12.541000, 0.375000)
(13.952982, 0.156250)
(19.874964, 0.062500)
(36.316109, 1.000000)
(14.172893, 0.312500)
(8.225883, 0.906250)
(13.984437, 0.000000)
(32.250385, 0.687500)
(20.073103, 0.312500)
(18.860682, 0.062500)
(21.450701, 0.093750)
(12.890105, 0.250000)
(20.801798, 0.000000)
(20.644512, 0.125000)
(19.323544, 0.218750)
(12.121391, 0.062500)
(15.076665, 0.187500)
(15.545311, 0.125000)
(15.126464, 0.000000)
(8.966540, 0.593750)
(14.076862, 0.093750)
(18.888176, 0.250000)
(12.218390, 0.250000)
(27.091944, 0.312500)
(8.184272, 0.750000)
(21.078032, 0.281250)
(34.766178, 0.843750)
(24.455320, 0.781250)
(9.089629, 0.656250)
(18.335535, 0.187500)
(10.185403, 0.250000)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_oampW_2.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 0.093750)
(17.552568, 0.312500)
(18.638512, 0.062500)
(18.546717, 0.093750)
(13.428638, 0.437500)
(16.794140, 0.156250)
(14.297143, 0.562500)
(17.171722, 0.281250)
(20.059292, 0.031250)
(11.256145, 0.781250)
(25.958267, 0.062500)
(14.636854, 0.125000)
(16.587755, 0.531250)
(8.500388, 0.812500)
(19.118383, 0.187500)
(19.355614, 0.000000)
(16.919485, 0.093750)
(10.740816, 0.718750)
(24.433674, 0.062500)
(15.328254, 0.375000)
(15.667542, 0.062500)
(32.651962, 0.000000)
(14.833853, 0.218750)
(24.772644, 0.000000)
(19.206205, 0.000000)
(18.807907, 0.062500)
(20.472019, 0.187500)
(24.486319, 0.000000)
(13.134361, 0.468750)
(14.394195, 0.625000)
(16.070848, 0.437500)
(25.167027, 0.000000)
(15.581610, 0.250000)
(17.096106, 0.187500)
(21.280998, 0.062500)
(23.876585, 0.062500)
(13.036207, 0.406250)
(22.731215, 0.000000)
(35.325077, 0.000000)
(24.573538, 0.062500)
(22.238827, 0.031250)
(17.241997, 0.093750)
(21.504358, 0.031250)
(16.334728, 0.156250)
(18.660828, 0.062500)
(10.326597, 0.875000)
(16.468248, 0.156250)
(13.946894, 0.500000)
(33.479321, 0.000000)
(13.391328, 0.156250)
(16.313137, 0.250000)
(17.417023, 0.125000)
(14.955702, 0.031250)
(23.593338, 0.125000)
(25.343109, 0.000000)
(28.576508, 0.000000)
(26.743855, 0.000000)
(17.670483, 0.343750)
(14.859500, 0.125000)
(13.146446, 0.250000)
(16.851610, 0.187500)
(24.674076, 0.000000)
(14.513160, 0.187500)
(18.443485, 0.156250)
(13.139583, 0.125000)
(13.289401, 0.562500)
(13.496741, 0.593750)
(17.107384, 0.375000)
(9.916093, 0.937500)
(12.541000, 0.500000)
(13.952982, 0.281250)
(19.874964, 0.031250)
(36.316109, 0.187500)
(14.172893, 0.437500)
(8.225883, 0.968750)
(13.984437, 0.187500)
(32.250385, 0.062500)
(20.073103, 0.062500)
(18.860682, 0.000000)
(21.450701, 0.000000)
(12.890105, 0.375000)
(20.801798, 0.000000)
(20.644512, 0.062500)
(19.323544, 0.000000)
(12.121391, 0.156250)
(15.076665, 0.375000)
(15.545311, 0.156250)
(15.126464, 0.062500)
(8.966540, 0.875000)
(14.076862, 0.250000)
(18.888176, 0.000000)
(12.218390, 0.437500)
(27.091944, 0.000000)
(8.184272, 0.937500)
(21.078032, 0.343750)
(34.766178, 0.093750)
(24.455320, 0.062500)
(9.089629, 0.843750)
(18.335535, 0.187500)
(10.185403, 0.812500)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_oampW_3.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 0.125000)
(17.552568, 0.312500)
(18.638512, 0.062500)
(18.546717, 0.156250)
(13.428638, 0.625000)
(16.794140, 0.125000)
(14.297143, 0.812500)
(17.171722, 0.250000)
(20.059292, 0.031250)
(11.256145, 0.750000)
(25.958267, 0.062500)
(14.636854, 0.125000)
(16.587755, 0.593750)
(8.500388, 0.812500)
(19.118383, 0.062500)
(19.355614, 0.000000)
(16.919485, 0.312500)
(10.740816, 0.750000)
(24.433674, 0.062500)
(15.328254, 0.437500)
(15.667542, 0.125000)
(32.651962, 0.000000)
(14.833853, 0.250000)
(24.772644, 0.000000)
(19.206205, 0.000000)
(18.807907, 0.062500)
(20.472019, 0.187500)
(24.486319, 0.000000)
(13.134361, 0.437500)
(14.394195, 0.625000)
(16.070848, 0.437500)
(25.167027, 0.000000)
(15.581610, 0.375000)
(17.096106, 0.187500)
(21.280998, 0.000000)
(23.876585, 0.031250)
(13.036207, 0.468750)
(22.731215, 0.000000)
(35.325077, 0.000000)
(24.573538, 0.062500)
(22.238827, 0.000000)
(17.241997, 0.062500)
(21.504358, 0.062500)
(16.334728, 0.187500)
(18.660828, 0.062500)
(10.326597, 0.875000)
(16.468248, 0.218750)
(13.946894, 0.500000)
(33.479321, 0.000000)
(13.391328, 0.281250)
(16.313137, 0.312500)
(17.417023, 0.125000)
(14.955702, 0.156250)
(23.593338, 0.125000)
(25.343109, 0.000000)
(28.576508, 0.000000)
(26.743855, 0.000000)
(17.670483, 0.343750)
(14.859500, 0.187500)
(13.146446, 0.250000)
(16.851610, 0.312500)
(24.674076, 0.000000)
(14.513160, 0.187500)
(18.443485, 0.156250)
(13.139583, 0.406250)
(13.289401, 0.625000)
(13.496741, 0.625000)
(17.107384, 0.500000)
(9.916093, 0.937500)
(12.541000, 0.562500)
(13.952982, 0.343750)
(19.874964, 0.031250)
(36.316109, 0.031250)
(14.172893, 0.468750)
(8.225883, 1.000000)
(13.984437, 0.218750)
(32.250385, 0.000000)
(20.073103, 0.125000)
(18.860682, 0.000000)
(21.450701, 0.000000)
(12.890105, 0.406250)
(20.801798, 0.000000)
(20.644512, 0.062500)
(19.323544, 0.000000)
(12.121391, 0.156250)
(15.076665, 0.468750)
(15.545311, 0.156250)
(15.126464, 0.093750)
(8.966540, 0.875000)
(14.076862, 0.312500)
(18.888176, 0.000000)
(12.218390, 0.468750)
(27.091944, 0.000000)
(8.184272, 0.968750)
(21.078032, 0.312500)
(34.766178, 0.000000)
(24.455320, 0.062500)
(9.089629, 0.843750)
(18.335535, 0.156250)
(10.185403, 0.906250)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_oampW_5.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 0.156250)
(17.552568, 0.375000)
(18.638512, 0.218750)
(18.546717, 0.187500)
(13.428638, 0.656250)
(16.794140, 0.187500)
(14.297143, 0.875000)
(17.171722, 0.281250)
(20.059292, 0.031250)
(11.256145, 0.750000)
(25.958267, 0.062500)
(14.636854, 0.218750)
(16.587755, 0.562500)
(8.500388, 0.812500)
(19.118383, 0.062500)
(19.355614, 0.000000)
(16.919485, 0.437500)
(10.740816, 0.937500)
(24.433674, 0.062500)
(15.328254, 0.468750)
(15.667542, 0.187500)
(32.651962, 0.000000)
(14.833853, 0.343750)
(24.772644, 0.000000)
(19.206205, 0.031250)
(18.807907, 0.125000)
(20.472019, 0.218750)
(24.486319, 0.000000)
(13.134361, 0.531250)
(14.394195, 0.718750)
(16.070848, 0.437500)
(25.167027, 0.031250)
(15.581610, 0.437500)
(17.096106, 0.218750)
(21.280998, 0.031250)
(23.876585, 0.031250)
(13.036207, 0.468750)
(22.731215, 0.000000)
(35.325077, 0.000000)
(24.573538, 0.062500)
(22.238827, 0.000000)
(17.241997, 0.156250)
(21.504358, 0.062500)
(16.334728, 0.250000)
(18.660828, 0.062500)
(10.326597, 0.875000)
(16.468248, 0.250000)
(13.946894, 0.500000)
(33.479321, 0.000000)
(13.391328, 0.468750)
(16.313137, 0.375000)
(17.417023, 0.125000)
(14.955702, 0.218750)
(23.593338, 0.187500)
(25.343109, 0.000000)
(28.576508, 0.062500)
(26.743855, 0.000000)
(17.670483, 0.375000)
(14.859500, 0.187500)
(13.146446, 0.406250)
(16.851610, 0.375000)
(24.674076, 0.000000)
(14.513160, 0.250000)
(18.443485, 0.187500)
(13.139583, 0.687500)
(13.289401, 0.656250)
(13.496741, 0.750000)
(17.107384, 0.562500)
(9.916093, 0.937500)
(12.541000, 0.562500)
(13.952982, 0.406250)
(19.874964, 0.062500)
(36.316109, 0.000000)
(14.172893, 0.531250)
(8.225883, 1.000000)
(13.984437, 0.343750)
(32.250385, 0.000000)
(20.073103, 0.156250)
(18.860682, 0.031250)
(21.450701, 0.031250)
(12.890105, 0.406250)
(20.801798, 0.031250)
(20.644512, 0.125000)
(19.323544, 0.031250)
(12.121391, 0.187500)
(15.076665, 0.468750)
(15.545311, 0.250000)
(15.126464, 0.156250)
(8.966540, 0.875000)
(14.076862, 0.312500)
(18.888176, 0.031250)
(12.218390, 0.500000)
(27.091944, 0.000000)
(8.184272, 1.000000)
(21.078032, 0.343750)
(34.766178, 0.000000)
(24.455320, 0.062500)
(9.089629, 0.875000)
(18.335535, 0.187500)
(10.185403, 0.937500)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_oampW_6.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 0.187500)
(17.552568, 0.375000)
(18.638512, 0.218750)
(18.546717, 0.218750)
(13.428638, 0.625000)
(16.794140, 0.156250)
(14.297143, 0.875000)
(17.171722, 0.250000)
(20.059292, 0.062500)
(11.256145, 0.781250)
(25.958267, 0.062500)
(14.636854, 0.312500)
(16.587755, 0.656250)
(8.500388, 0.812500)
(19.118383, 0.062500)
(19.355614, 0.000000)
(16.919485, 0.500000)
(10.740816, 0.843750)
(24.433674, 0.093750)
(15.328254, 0.437500)
(15.667542, 0.156250)
(32.651962, 0.000000)
(14.833853, 0.312500)
(24.772644, 0.000000)
(19.206205, 0.062500)
(18.807907, 0.093750)
(20.472019, 0.250000)
(24.486319, 0.000000)
(13.134361, 0.531250)
(14.394195, 0.750000)
(16.070848, 0.437500)
(25.167027, 0.031250)
(15.581610, 0.437500)
(17.096106, 0.218750)
(21.280998, 0.031250)
(23.876585, 0.031250)
(13.036207, 0.468750)
(22.731215, 0.000000)
(35.325077, 0.000000)
(24.573538, 0.062500)
(22.238827, 0.000000)
(17.241997, 0.062500)
(21.504358, 0.093750)
(16.334728, 0.187500)
(18.660828, 0.093750)
(10.326597, 0.875000)
(16.468248, 0.218750)
(13.946894, 0.500000)
(33.479321, 0.000000)
(13.391328, 0.437500)
(16.313137, 0.343750)
(17.417023, 0.125000)
(14.955702, 0.156250)
(23.593338, 0.187500)
(25.343109, 0.000000)
(28.576508, 0.000000)
(26.743855, 0.031250)
(17.670483, 0.437500)
(14.859500, 0.125000)
(13.146446, 0.406250)
(16.851610, 0.281250)
(24.674076, 0.000000)
(14.513160, 0.218750)
(18.443485, 0.187500)
(13.139583, 0.500000)
(13.289401, 0.656250)
(13.496741, 0.781250)
(17.107384, 0.562500)
(9.916093, 0.937500)
(12.541000, 0.562500)
(13.952982, 0.375000)
(19.874964, 0.062500)
(36.316109, 0.000000)
(14.172893, 0.437500)
(8.225883, 1.000000)
(13.984437, 0.343750)
(32.250385, 0.000000)
(20.073103, 0.156250)
(18.860682, 0.031250)
(21.450701, 0.031250)
(12.890105, 0.343750)
(20.801798, 0.000000)
(20.644512, 0.093750)
(19.323544, 0.031250)
(12.121391, 0.187500)
(15.076665, 0.531250)
(15.545311, 0.218750)
(15.126464, 0.156250)
(8.966540, 0.875000)
(14.076862, 0.312500)
(18.888176, 0.031250)
(12.218390, 0.500000)
(27.091944, 0.000000)
(8.184272, 0.968750)
(21.078032, 0.343750)
(34.766178, 0.000000)
(24.455320, 0.062500)
(9.089629, 0.843750)
(18.335535, 0.187500)
(10.185403, 0.937500)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_oampW_7.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 0.187500)
(17.552568, 0.375000)
(18.638512, 0.156250)
(18.546717, 0.156250)
(13.428638, 0.531250)
(16.794140, 0.156250)
(14.297143, 0.750000)
(17.171722, 0.250000)
(20.059292, 0.031250)
(11.256145, 0.781250)
(25.958267, 0.062500)
(14.636854, 0.218750)
(16.587755, 0.531250)
(8.500388, 0.687500)
(19.118383, 0.062500)
(19.355614, 0.000000)
(16.919485, 0.437500)
(10.740816, 0.781250)
(24.433674, 0.062500)
(15.328254, 0.437500)
(15.667542, 0.093750)
(32.651962, 0.000000)
(14.833853, 0.312500)
(24.772644, 0.000000)
(19.206205, 0.093750)
(18.807907, 0.062500)
(20.472019, 0.187500)
(24.486319, 0.000000)
(13.134361, 0.562500)
(14.394195, 0.687500)
(16.070848, 0.437500)
(25.167027, 0.031250)
(15.581610, 0.437500)
(17.096106, 0.187500)
(21.280998, 0.031250)
(23.876585, 0.031250)
(13.036207, 0.468750)
(22.731215, 0.000000)
(35.325077, 0.000000)
(24.573538, 0.062500)
(22.238827, 0.000000)
(17.241997, 0.062500)
(21.504358, 0.062500)
(16.334728, 0.250000)
(18.660828, 0.125000)
(10.326597, 0.875000)
(16.468248, 0.218750)
(13.946894, 0.500000)
(33.479321, 0.000000)
(13.391328, 0.375000)
(16.313137, 0.343750)
(17.417023, 0.156250)
(14.955702, 0.093750)
(23.593338, 0.125000)
(25.343109, 0.000000)
(28.576508, 0.031250)
(26.743855, 0.000000)
(17.670483, 0.625000)
(14.859500, 0.187500)
(13.146446, 0.343750)
(16.851610, 0.312500)
(24.674076, 0.000000)
(14.513160, 0.218750)
(18.443485, 0.187500)
(13.139583, 0.531250)
(13.289401, 0.625000)
(13.496741, 0.750000)
(17.107384, 0.687500)
(9.916093, 0.937500)
(12.541000, 0.531250)
(13.952982, 0.312500)
(19.874964, 0.062500)
(36.316109, 0.000000)
(14.172893, 0.500000)
(8.225883, 1.000000)
(13.984437, 0.250000)
(32.250385, 0.000000)
(20.073103, 0.125000)
(18.860682, 0.031250)
(21.450701, 0.031250)
(12.890105, 0.406250)
(20.801798, 0.000000)
(20.644512, 0.125000)
(19.323544, 0.000000)
(12.121391, 0.125000)
(15.076665, 0.468750)
(15.545311, 0.281250)
(15.126464, 0.156250)
(8.966540, 0.781250)
(14.076862, 0.312500)
(18.888176, 0.031250)
(12.218390, 0.500000)
(27.091944, 0.000000)
(8.184272, 0.937500)
(21.078032, 0.250000)
(34.766178, 0.000000)
(24.455320, 0.062500)
(9.089629, 0.875000)
(18.335535, 0.187500)
(10.185403, 0.875000)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_oampW_8.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 0.156250)
(17.552568, 0.375000)
(18.638512, 0.156250)
(18.546717, 0.218750)
(13.428638, 0.656250)
(16.794140, 0.156250)
(14.297143, 0.937500)
(17.171722, 0.250000)
(20.059292, 0.031250)
(11.256145, 0.781250)
(25.958267, 0.062500)
(14.636854, 0.218750)
(16.587755, 0.593750)
(8.500388, 0.812500)
(19.118383, 0.062500)
(19.355614, 0.000000)
(16.919485, 0.406250)
(10.740816, 0.937500)
(24.433674, 0.062500)
(15.328254, 0.437500)
(15.667542, 0.218750)
(32.651962, 0.000000)
(14.833853, 0.312500)
(24.772644, 0.000000)
(19.206205, 0.062500)
(18.807907, 0.093750)
(20.472019, 0.250000)
(24.486319, 0.000000)
(13.134361, 0.593750)
(14.394195, 0.687500)
(16.070848, 0.437500)
(25.167027, 0.031250)
(15.581610, 0.375000)
(17.096106, 0.218750)
(21.280998, 0.031250)
(23.876585, 0.031250)
(13.036207, 0.500000)
(22.731215, 0.000000)
(35.325077, 0.000000)
(24.573538, 0.062500)
(22.238827, 0.000000)
(17.241997, 0.062500)
(21.504358, 0.031250)
(16.334728, 0.187500)
(18.660828, 0.062500)
(10.326597, 0.875000)
(16.468248, 0.250000)
(13.946894, 0.500000)
(33.479321, 0.000000)
(13.391328, 0.406250)
(16.313137, 0.343750)
(17.417023, 0.156250)
(14.955702, 0.187500)
(23.593338, 0.125000)
(25.343109, 0.000000)
(28.576508, 0.000000)
(26.743855, 0.000000)
(17.670483, 0.406250)
(14.859500, 0.187500)
(13.146446, 0.343750)
(16.851610, 0.250000)
(24.674076, 0.000000)
(14.513160, 0.218750)
(18.443485, 0.187500)
(13.139583, 0.625000)
(13.289401, 0.625000)
(13.496741, 0.750000)
(17.107384, 0.531250)
(9.916093, 0.937500)
(12.541000, 0.562500)
(13.952982, 0.343750)
(19.874964, 0.031250)
(36.316109, 0.000000)
(14.172893, 0.468750)
(8.225883, 0.937500)
(13.984437, 0.375000)
(32.250385, 0.000000)
(20.073103, 0.125000)
(18.860682, 0.031250)
(21.450701, 0.031250)
(12.890105, 0.343750)
(20.801798, 0.031250)
(20.644512, 0.093750)
(19.323544, 0.000000)
(12.121391, 0.187500)
(15.076665, 0.375000)
(15.545311, 0.281250)
(15.126464, 0.156250)
(8.966540, 0.875000)
(14.076862, 0.250000)
(18.888176, 0.031250)
(12.218390, 0.500000)
(27.091944, 0.000000)
(8.184272, 0.937500)
(21.078032, 0.312500)
(34.766178, 0.000000)
(24.455320, 0.031250)
(9.089629, 0.843750)
(18.335535, 0.187500)
(10.185403, 0.937500)
};


==> figures/rawfiles/Gaussianratiovscond/Gaussianratiovscond_oampW_9.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 0.156250)
(17.552568, 0.375000)
(18.638512, 0.187500)
(18.546717, 0.218750)
(13.428638, 0.781250)
(16.794140, 0.156250)
(14.297143, 0.937500)
(17.171722, 0.281250)
(20.059292, 0.062500)
(11.256145, 0.781250)
(25.958267, 0.062500)
(14.636854, 0.250000)
(16.587755, 0.718750)
(8.500388, 0.843750)
(19.118383, 0.093750)
(19.355614, 0.000000)
(16.919485, 0.562500)
(10.740816, 0.937500)
(24.433674, 0.062500)
(15.328254, 0.437500)
(15.667542, 0.218750)
(32.651962, 0.000000)
(14.833853, 0.531250)
(24.772644, 0.000000)
(19.206205, 0.062500)
(18.807907, 0.156250)
(20.472019, 0.250000)
(24.486319, 0.000000)
(13.134361, 0.656250)
(14.394195, 0.750000)
(16.070848, 0.437500)
(25.167027, 0.031250)
(15.581610, 0.437500)
(17.096106, 0.343750)
(21.280998, 0.031250)
(23.876585, 0.031250)
(13.036207, 0.531250)
(22.731215, 0.000000)
(35.325077, 0.000000)
(24.573538, 0.062500)
(22.238827, 0.000000)
(17.241997, 0.062500)
(21.504358, 0.031250)
(16.334728, 0.281250)
(18.660828, 0.062500)
(10.326597, 0.937500)
(16.468248, 0.406250)
(13.946894, 0.500000)
(33.479321, 0.000000)
(13.391328, 0.468750)
(16.313137, 0.343750)
(17.417023, 0.156250)
(14.955702, 0.312500)
(23.593338, 0.125000)
(25.343109, 0.000000)
(28.576508, 0.031250)
(26.743855, 0.000000)
(17.670483, 0.468750)
(14.859500, 0.250000)
(13.146446, 0.375000)
(16.851610, 0.343750)
(24.674076, 0.000000)
(14.513160, 0.312500)
(18.443485, 0.187500)
(13.139583, 0.687500)
(13.289401, 0.718750)
(13.496741, 0.656250)
(17.107384, 0.687500)
(9.916093, 0.937500)
(12.541000, 0.593750)
(13.952982, 0.375000)
(19.874964, 0.062500)
(36.316109, 0.000000)
(14.172893, 0.531250)
(8.225883, 1.000000)
(13.984437, 0.375000)
(32.250385, 0.000000)
(20.073103, 0.187500)
(18.860682, 0.031250)
(21.450701, 0.031250)
(12.890105, 0.437500)
(20.801798, 0.062500)
(20.644512, 0.093750)
(19.323544, 0.000000)
(12.121391, 0.218750)
(15.076665, 0.562500)
(15.545311, 0.312500)
(15.126464, 0.156250)
(8.966540, 0.875000)
(14.076862, 0.312500)
(18.888176, 0.031250)
(12.218390, 0.500000)
(27.091944, 0.000000)
(8.184272, 1.000000)
(21.078032, 0.375000)
(34.766178, 0.000000)
(24.455320, 0.031250)
(9.089629, 0.875000)
(18.335535, 0.187500)
(10.185403, 0.937500)
};


==> figures/rawfiles/anderson_score_cdf/hist_layer0_learnW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.001565)
(0.120679, 0.020031)
(0.145635, 0.052895)
(0.175751, 0.119562)
(0.212095, 0.227230)
(0.255955, 0.351800)
(0.308884, 0.500782)
(0.372759, 0.636933)
(0.449843, 0.763693)
(0.542868, 0.853208)
(0.655129, 0.914241)
(0.790604, 0.951487)
(0.954095, 0.969014)
(1.151395, 0.978404)
(1.389495, 0.984664)
(1.676833, 0.988732)
(2.023590, 0.991549)
(2.442053, 0.994366)
(2.947052, 0.995931)
(3.556480, 0.996870)
(4.291934, 0.998122)
(5.179475, 0.998435)
(6.250552, 0.998748)
(7.543120, 0.998748)
(9.102982, 0.999687)
(10.985411, 1.000000)
(13.257114, 1.000000)
(15.998587, 1.000000)
(19.306977, 1.000000)
(23.299518, 1.000000)
(28.117687, 1.000000)
(33.932218, 1.000000)
(40.949151, 1.000000)
(49.417134, 1.000000)
(59.636233, 1.000000)
(71.968567, 1.000000)
(86.851137, 1.000000)
(104.811313, 1.000000)
(126.485522, 1.000000)
(152.641797, 1.000000)
(184.206997, 1.000000)
(222.299648, 1.000000)
(268.269580, 1.000000)
(323.745754, 1.000000)
(390.693994, 1.000000)
(471.486636, 1.000000)
(568.986603, 1.000000)
(686.648845, 1.000000)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer0_oampW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.004382)
(0.120679, 0.017214)
(0.145635, 0.047574)
(0.175751, 0.114241)
(0.212095, 0.213772)
(0.255955, 0.334898)
(0.308884, 0.482942)
(0.372759, 0.609703)
(0.449843, 0.711111)
(0.542868, 0.806573)
(0.655129, 0.868858)
(0.790604, 0.908294)
(0.954095, 0.933646)
(1.151395, 0.946166)
(1.389495, 0.953678)
(1.676833, 0.961815)
(2.023590, 0.969014)
(2.442053, 0.975587)
(2.947052, 0.979969)
(3.556480, 0.983099)
(4.291934, 0.986854)
(5.179475, 0.988732)
(6.250552, 0.992488)
(7.543120, 0.994679)
(9.102982, 0.996557)
(10.985411, 0.997809)
(13.257114, 0.999374)
(15.998587, 0.999687)
(19.306977, 1.000000)
(23.299518, 1.000000)
(28.117687, 1.000000)
(33.932218, 1.000000)
(40.949151, 1.000000)
(49.417134, 1.000000)
(59.636233, 1.000000)
(71.968567, 1.000000)
(86.851137, 1.000000)
(104.811313, 1.000000)
(126.485522, 1.000000)
(152.641797, 1.000000)
(184.206997, 1.000000)
(222.299648, 1.000000)
(268.269580, 1.000000)
(323.745754, 1.000000)
(390.693994, 1.000000)
(471.486636, 1.000000)
(568.986603, 1.000000)
(686.648845, 1.000000)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer1_learnW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.000313)
(0.120679, 0.001875)
(0.145635, 0.006562)
(0.175751, 0.017500)
(0.212095, 0.035625)
(0.255955, 0.058438)
(0.308884, 0.097188)
(0.372759, 0.138750)
(0.449843, 0.195625)
(0.542868, 0.256875)
(0.655129, 0.313438)
(0.790604, 0.370625)
(0.954095, 0.440625)
(1.151395, 0.509063)
(1.389495, 0.564375)
(1.676833, 0.612813)
(2.023590, 0.664688)
(2.442053, 0.713438)
(2.947052, 0.756250)
(3.556480, 0.796875)
(4.291934, 0.837188)
(5.179475, 0.868750)
(6.250552, 0.895313)
(7.543120, 0.917188)
(9.102982, 0.936875)
(10.985411, 0.955938)
(13.257114, 0.965938)
(15.998587, 0.976250)
(19.306977, 0.981563)
(23.299518, 0.988750)
(28.117687, 0.992813)
(33.932218, 0.995313)
(40.949151, 0.997188)
(49.417134, 0.998125)
(59.636233, 0.999063)
(71.968567, 1.000000)
(86.851137, 1.000000)
(104.811313, 1.000000)
(126.485522, 1.000000)
(152.641797, 1.000000)
(184.206997, 1.000000)
(222.299648, 1.000000)
(268.269580, 1.000000)
(323.745754, 1.000000)
(390.693994, 1.000000)
(471.486636, 1.000000)
(568.986603, 1.000000)
(686.648845, 1.000000)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer1_oampW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.000000)
(0.120679, 0.000000)
(0.145635, 0.000313)
(0.175751, 0.000937)
(0.212095, 0.002500)
(0.255955, 0.007500)
(0.308884, 0.012812)
(0.372759, 0.019062)
(0.449843, 0.025313)
(0.542868, 0.033125)
(0.655129, 0.048125)
(0.790604, 0.063438)
(0.954095, 0.079375)
(1.151395, 0.093750)
(1.389495, 0.115625)
(1.676833, 0.136875)
(2.023590, 0.158125)
(2.442053, 0.184062)
(2.947052, 0.219375)
(3.556480, 0.247812)
(4.291934, 0.277812)
(5.179475, 0.313125)
(6.250552, 0.357500)
(7.543120, 0.397500)
(9.102982, 0.440000)
(10.985411, 0.492500)
(13.257114, 0.532500)
(15.998587, 0.581875)
(19.306977, 0.627500)
(23.299518, 0.664062)
(28.117687, 0.710313)
(33.932218, 0.749375)
(40.949151, 0.785625)
(49.417134, 0.825625)
(59.636233, 0.860313)
(71.968567, 0.886875)
(86.851137, 0.915938)
(104.811313, 0.937500)
(126.485522, 0.952813)
(152.641797, 0.965938)
(184.206997, 0.976563)
(222.299648, 0.985938)
(268.269580, 0.990625)
(323.745754, 0.995313)
(390.693994, 0.996563)
(471.486636, 0.998750)
(568.986603, 1.000000)
(686.648845, 1.000000)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer2_learnW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.000313)
(0.120679, 0.003440)
(0.145635, 0.017824)
(0.175751, 0.042839)
(0.212095, 0.077861)
(0.255955, 0.133521)
(0.308884, 0.200125)
(0.372759, 0.267980)
(0.449843, 0.337086)
(0.542868, 0.410882)
(0.655129, 0.475297)
(0.790604, 0.531582)
(0.954095, 0.577236)
(1.151395, 0.622889)
(1.389495, 0.658849)
(1.676833, 0.696685)
(2.023590, 0.727017)
(2.442053, 0.759537)
(2.947052, 0.793621)
(3.556480, 0.824578)
(4.291934, 0.848343)
(5.179475, 0.873358)
(6.250552, 0.893371)
(7.543120, 0.912133)
(9.102982, 0.927767)
(10.985411, 0.943089)
(13.257114, 0.955597)
(15.998587, 0.965916)
(19.306977, 0.974672)
(23.299518, 0.983740)
(28.117687, 0.988430)
(33.932218, 0.990306)
(40.949151, 0.993121)
(49.417134, 0.995310)
(59.636233, 0.997186)
(71.968567, 0.998124)
(86.851137, 0.999062)
(104.811313, 0.999687)
(126.485522, 1.000000)
(152.641797, 1.000000)
(184.206997, 1.000000)
(222.299648, 1.000000)
(268.269580, 1.000000)
(323.745754, 1.000000)
(390.693994, 1.000000)
(471.486636, 1.000000)
(568.986603, 1.000000)
(686.648845, 1.000000)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer2_oampW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.000000)
(0.120679, 0.000625)
(0.145635, 0.002500)
(0.175751, 0.005000)
(0.212095, 0.009062)
(0.255955, 0.016250)
(0.308884, 0.023750)
(0.372759, 0.034375)
(0.449843, 0.048125)
(0.542868, 0.060625)
(0.655129, 0.069687)
(0.790604, 0.080312)
(0.954095, 0.093437)
(1.151395, 0.109375)
(1.389495, 0.124375)
(1.676833, 0.144687)
(2.023590, 0.163437)
(2.442053, 0.180937)
(2.947052, 0.204687)
(3.556480, 0.221875)
(4.291934, 0.245625)
(5.179475, 0.271250)
(6.250552, 0.299687)
(7.543120, 0.328750)
(9.102982, 0.355000)
(10.985411, 0.385625)
(13.257114, 0.417500)
(15.998587, 0.454687)
(19.306977, 0.490000)
(23.299518, 0.529375)
(28.117687, 0.572500)
(33.932218, 0.608750)
(40.949151, 0.645312)
(49.417134, 0.687187)
(59.636233, 0.723437)
(71.968567, 0.753125)
(86.851137, 0.785937)
(104.811313, 0.816250)
(126.485522, 0.848437)
(152.641797, 0.872812)
(184.206997, 0.897813)
(222.299648, 0.922500)
(268.269580, 0.941250)
(323.745754, 0.956562)
(390.693994, 0.975938)
(471.486636, 0.988437)
(568.986603, 0.995000)
(686.648845, 0.999375)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer3_learnW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.002502)
(0.120679, 0.010944)
(0.145635, 0.024390)
(0.175751, 0.060038)
(0.212095, 0.120388)
(0.255955, 0.206066)
(0.308884, 0.310194)
(0.372759, 0.413071)
(0.449843, 0.505629)
(0.542868, 0.586929)
(0.655129, 0.643840)
(0.790604, 0.693871)
(0.954095, 0.729206)
(1.151395, 0.758912)
(1.389495, 0.786429)
(1.676833, 0.807380)
(2.023590, 0.830519)
(2.442053, 0.852095)
(2.947052, 0.865854)
(3.556480, 0.881801)
(4.291934, 0.897123)
(5.179475, 0.912445)
(6.250552, 0.925266)
(7.543120, 0.941213)
(9.102982, 0.949969)
(10.985411, 0.958724)
(13.257114, 0.966854)
(15.998587, 0.972795)
(19.306977, 0.979675)
(23.299518, 0.984678)
(28.117687, 0.989368)
(33.932218, 0.992808)
(40.949151, 0.994684)
(49.417134, 0.996873)
(59.636233, 0.998437)
(71.968567, 0.999062)
(86.851137, 0.999687)
(104.811313, 1.000000)
(126.485522, 1.000000)
(152.641797, 1.000000)
(184.206997, 1.000000)
(222.299648, 1.000000)
(268.269580, 1.000000)
(323.745754, 1.000000)
(390.693994, 1.000000)
(471.486636, 1.000000)
(568.986603, 1.000000)
(686.648845, 1.000000)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer3_oampW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.000000)
(0.120679, 0.000313)
(0.145635, 0.003125)
(0.175751, 0.005000)
(0.212095, 0.009375)
(0.255955, 0.018750)
(0.308884, 0.028125)
(0.372759, 0.039375)
(0.449843, 0.054375)
(0.542868, 0.067500)
(0.655129, 0.080938)
(0.790604, 0.091563)
(0.954095, 0.104688)
(1.151395, 0.126250)
(1.389495, 0.147813)
(1.676833, 0.165313)
(2.023590, 0.183125)
(2.442053, 0.201563)
(2.947052, 0.222500)
(3.556480, 0.242188)
(4.291934, 0.267188)
(5.179475, 0.289062)
(6.250552, 0.315937)
(7.543120, 0.340625)
(9.102982, 0.371875)
(10.985411, 0.401250)
(13.257114, 0.426562)
(15.998587, 0.459062)
(19.306977, 0.494687)
(23.299518, 0.529687)
(28.117687, 0.563750)
(33.932218, 0.603437)
(40.949151, 0.641875)
(49.417134, 0.679688)
(59.636233, 0.714688)
(71.968567, 0.746875)
(86.851137, 0.773438)
(104.811313, 0.800625)
(126.485522, 0.825938)
(152.641797, 0.857813)
(184.206997, 0.882188)
(222.299648, 0.909688)
(268.269580, 0.929375)
(323.745754, 0.948125)
(390.693994, 0.964375)
(471.486636, 0.983438)
(568.986603, 0.991875)
(686.648845, 0.997813)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer4_learnW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.002188)
(0.120679, 0.010941)
(0.145635, 0.031260)
(0.175751, 0.079400)
(0.212095, 0.150672)
(0.255955, 0.241638)
(0.308884, 0.351047)
(0.372759, 0.467021)
(0.449843, 0.578618)
(0.542868, 0.656143)
(0.655129, 0.718662)
(0.790604, 0.765864)
(0.954095, 0.799312)
(1.151395, 0.823382)
(1.389495, 0.841200)
(1.676833, 0.859018)
(2.023590, 0.873711)
(2.442053, 0.890591)
(2.947052, 0.904345)
(3.556480, 0.914661)
(4.291934, 0.929040)
(5.179475, 0.945921)
(6.250552, 0.954986)
(7.543120, 0.963113)
(9.102982, 0.968428)
(10.985411, 0.972804)
(13.257114, 0.977493)
(15.998587, 0.982182)
(19.306977, 0.985933)
(23.299518, 0.990935)
(28.117687, 0.994998)
(33.932218, 0.997187)
(40.949151, 0.997499)
(49.417134, 0.998437)
(59.636233, 0.998750)
(71.968567, 0.998750)
(86.851137, 0.998750)
(104.811313, 0.998750)
(126.485522, 0.999375)
(152.641797, 0.999375)
(184.206997, 0.999687)
(222.299648, 1.000000)
(268.269580, 1.000000)
(323.745754, 1.000000)
(390.693994, 1.000000)
(471.486636, 1.000000)
(568.986603, 1.000000)
(686.648845, 1.000000)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer4_oampW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.000000)
(0.120679, 0.000625)
(0.145635, 0.002187)
(0.175751, 0.005625)
(0.212095, 0.009687)
(0.255955, 0.019063)
(0.308884, 0.033750)
(0.372759, 0.049063)
(0.449843, 0.063125)
(0.542868, 0.078437)
(0.655129, 0.098125)
(0.790604, 0.114375)
(0.954095, 0.129687)
(1.151395, 0.155937)
(1.389495, 0.174062)
(1.676833, 0.191562)
(2.023590, 0.212500)
(2.442053, 0.230625)
(2.947052, 0.252500)
(3.556480, 0.274375)
(4.291934, 0.299687)
(5.179475, 0.327812)
(6.250552, 0.355312)
(7.543120, 0.384062)
(9.102982, 0.406875)
(10.985411, 0.431250)
(13.257114, 0.465000)
(15.998587, 0.493437)
(19.306977, 0.528750)
(23.299518, 0.563437)
(28.117687, 0.601250)
(33.932218, 0.639062)
(40.949151, 0.672187)
(49.417134, 0.701562)
(59.636233, 0.723750)
(71.968567, 0.749062)
(86.851137, 0.772187)
(104.811313, 0.805000)
(126.485522, 0.831250)
(152.641797, 0.859375)
(184.206997, 0.880312)
(222.299648, 0.899375)
(268.269580, 0.924687)
(323.745754, 0.943750)
(390.693994, 0.960625)
(471.486636, 0.977500)
(568.986603, 0.991250)
(686.648845, 0.997500)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer5_learnW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.004376)
(0.120679, 0.011879)
(0.145635, 0.037824)
(0.175751, 0.091904)
(0.212095, 0.167240)
(0.255955, 0.282901)
(0.308884, 0.397312)
(0.372759, 0.511410)
(0.449843, 0.614567)
(0.542868, 0.698031)
(0.655129, 0.755236)
(0.790604, 0.788371)
(0.954095, 0.823695)
(1.151395, 0.847765)
(1.389495, 0.868709)
(1.676833, 0.885589)
(2.023590, 0.899031)
(2.442053, 0.915599)
(2.947052, 0.929353)
(3.556480, 0.939356)
(4.291934, 0.945921)
(5.179475, 0.954048)
(6.250552, 0.963113)
(7.543120, 0.970928)
(9.102982, 0.976868)
(10.985411, 0.982182)
(13.257114, 0.986246)
(15.998587, 0.988434)
(19.306977, 0.992810)
(23.299518, 0.994373)
(28.117687, 0.995624)
(33.932218, 0.997812)
(40.949151, 0.998124)
(49.417134, 0.998750)
(59.636233, 0.999375)
(71.968567, 1.000000)
(86.851137, 1.000000)
(104.811313, 1.000000)
(126.485522, 1.000000)
(152.641797, 1.000000)
(184.206997, 1.000000)
(222.299648, 1.000000)
(268.269580, 1.000000)
(323.745754, 1.000000)
(390.693994, 1.000000)
(471.486636, 1.000000)
(568.986603, 1.000000)
(686.648845, 1.000000)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer5_oampW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.000000)
(0.120679, 0.000625)
(0.145635, 0.002500)
(0.175751, 0.005625)
(0.212095, 0.010937)
(0.255955, 0.023125)
(0.308884, 0.036875)
(0.372759, 0.050312)
(0.449843, 0.065625)
(0.542868, 0.083437)
(0.655129, 0.100312)
(0.790604, 0.115937)
(0.954095, 0.136875)
(1.151395, 0.155312)
(1.389495, 0.177812)
(1.676833, 0.200000)
(2.023590, 0.219062)
(2.442053, 0.237187)
(2.947052, 0.257188)
(3.556480, 0.281250)
(4.291934, 0.305000)
(5.179475, 0.327500)
(6.250552, 0.354063)
(7.543120, 0.379375)
(9.102982, 0.405313)
(10.985411, 0.434063)
(13.257114, 0.464062)
(15.998587, 0.497500)
(19.306977, 0.531563)
(23.299518, 0.560312)
(28.117687, 0.599687)
(33.932218, 0.632187)
(40.949151, 0.668437)
(49.417134, 0.698750)
(59.636233, 0.724687)
(71.968567, 0.750625)
(86.851137, 0.773750)
(104.811313, 0.800937)
(126.485522, 0.830937)
(152.641797, 0.853750)
(184.206997, 0.877187)
(222.299648, 0.897187)
(268.269580, 0.919062)
(323.745754, 0.940625)
(390.693994, 0.955000)
(471.486636, 0.973437)
(568.986603, 0.990312)
(686.648845, 0.996250)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer6_learnW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.002813)
(0.120679, 0.013129)
(0.145635, 0.045014)
(0.175751, 0.096280)
(0.212095, 0.178806)
(0.255955, 0.290091)
(0.308884, 0.413254)
(0.372759, 0.540481)
(0.449843, 0.645514)
(0.542868, 0.723351)
(0.655129, 0.777743)
(0.790604, 0.814942)
(0.954095, 0.844952)
(1.151395, 0.866208)
(1.389495, 0.879650)
(1.676833, 0.893092)
(2.023590, 0.908096)
(2.442053, 0.924351)
(2.947052, 0.936543)
(3.556480, 0.945608)
(4.291934, 0.952485)
(5.179475, 0.964364)
(6.250552, 0.971554)
(7.543120, 0.978118)
(9.102982, 0.979994)
(10.985411, 0.987496)
(13.257114, 0.991247)
(15.998587, 0.994061)
(19.306977, 0.995624)
(23.299518, 0.996561)
(28.117687, 0.997499)
(33.932218, 0.998124)
(40.949151, 0.998750)
(49.417134, 0.999375)
(59.636233, 1.000000)
(71.968567, 1.000000)
(86.851137, 1.000000)
(104.811313, 1.000000)
(126.485522, 1.000000)
(152.641797, 1.000000)
(184.206997, 1.000000)
(222.299648, 1.000000)
(268.269580, 1.000000)
(323.745754, 1.000000)
(390.693994, 1.000000)
(471.486636, 1.000000)
(568.986603, 1.000000)
(686.648845, 1.000000)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer6_oampW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.000000)
(0.120679, 0.000940)
(0.145635, 0.003132)
(0.175751, 0.005951)
(0.212095, 0.010022)
(0.255955, 0.020357)
(0.308884, 0.036016)
(0.372759, 0.050736)
(0.449843, 0.066395)
(0.542868, 0.084873)
(0.655129, 0.102725)
(0.790604, 0.118384)
(0.954095, 0.138741)
(1.151395, 0.160038)
(1.389495, 0.183840)
(1.676833, 0.201065)
(2.023590, 0.215785)
(2.442053, 0.234576)
(2.947052, 0.254306)
(3.556480, 0.279048)
(4.291934, 0.298779)
(5.179475, 0.324460)
(6.250552, 0.349515)
(7.543120, 0.378641)
(9.102982, 0.398998)
(10.985411, 0.429690)
(13.257114, 0.457250)
(15.998587, 0.485124)
(19.306977, 0.516755)
(23.299518, 0.547761)
(28.117687, 0.580332)
(33.932218, 0.610085)
(40.949151, 0.636392)
(49.417134, 0.661134)
(59.636233, 0.684936)
(71.968567, 0.710617)
(86.851137, 0.740996)
(104.811313, 0.771375)
(126.485522, 0.798935)
(152.641797, 0.823050)
(184.206997, 0.844973)
(222.299648, 0.871907)
(268.269580, 0.894457)
(323.745754, 0.919198)
(390.693994, 0.940182)
(471.486636, 0.957094)
(568.986603, 0.978703)
(686.648845, 0.989978)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer7_learnW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.002189)
(0.120679, 0.014384)
(0.145635, 0.042839)
(0.175751, 0.093183)
(0.212095, 0.177611)
(0.255955, 0.287680)
(0.308884, 0.413696)
(0.372759, 0.542839)
(0.449843, 0.640400)
(0.542868, 0.721388)
(0.655129, 0.786116)
(0.790604, 0.825516)
(0.954095, 0.853659)
(1.151395, 0.873984)
(1.389495, 0.892745)
(1.676833, 0.910256)
(2.023590, 0.922139)
(2.442053, 0.934021)
(2.947052, 0.946529)
(3.556480, 0.953721)
(4.291934, 0.963102)
(5.179475, 0.967480)
(6.250552, 0.974672)
(7.543120, 0.980300)
(9.102982, 0.984991)
(10.985411, 0.988118)
(13.257114, 0.990932)
(15.998587, 0.994684)
(19.306977, 0.996248)
(23.299518, 0.997186)
(28.117687, 0.997811)
(33.932218, 0.998437)
(40.949151, 0.999062)
(49.417134, 0.999375)
(59.636233, 0.999375)
(71.968567, 0.999375)
(86.851137, 0.999375)
(104.811313, 1.000000)
(126.485522, 1.000000)
(152.641797, 1.000000)
(184.206997, 1.000000)
(222.299648, 1.000000)
(268.269580, 1.000000)
(323.745754, 1.000000)
(390.693994, 1.000000)
(471.486636, 1.000000)
(568.986603, 1.000000)
(686.648845, 1.000000)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer7_oampW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.000000)
(0.120679, 0.001255)
(0.145635, 0.003137)
(0.175751, 0.006274)
(0.212095, 0.010038)
(0.255955, 0.018507)
(0.308884, 0.034504)
(0.372759, 0.048306)
(0.449843, 0.065872)
(0.542868, 0.082497)
(0.655129, 0.099435)
(0.790604, 0.114492)
(0.954095, 0.133312)
(1.151395, 0.153701)
(1.389495, 0.174404)
(1.676833, 0.191029)
(2.023590, 0.209536)
(2.442053, 0.227729)
(2.947052, 0.244354)
(3.556480, 0.267880)
(4.291934, 0.287014)
(5.179475, 0.307403)
(6.250552, 0.333124)
(7.543120, 0.356964)
(9.102982, 0.379548)
(10.985411, 0.407465)
(13.257114, 0.433501)
(15.998587, 0.456085)
(19.306977, 0.488080)
(23.299518, 0.513174)
(28.117687, 0.538896)
(33.932218, 0.566813)
(40.949151, 0.595671)
(49.417134, 0.624843)
(59.636233, 0.655270)
(71.968567, 0.681305)
(86.851137, 0.703262)
(104.811313, 0.734003)
(126.485522, 0.762861)
(152.641797, 0.792974)
(184.206997, 0.817127)
(222.299648, 0.842848)
(268.269580, 0.870765)
(323.745754, 0.899310)
(390.693994, 0.924090)
(471.486636, 0.942597)
(568.986603, 0.962359)
(686.648845, 0.984316)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer8_learnW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.002814)
(0.120679, 0.012821)
(0.145635, 0.041901)
(0.175751, 0.105378)
(0.212095, 0.189806)
(0.255955, 0.300500)
(0.308884, 0.421826)
(0.372759, 0.545341)
(0.449843, 0.653846)
(0.542868, 0.730144)
(0.655129, 0.792996)
(0.790604, 0.828956)
(0.954095, 0.859600)
(1.151395, 0.884615)
(1.389495, 0.902126)
(1.676833, 0.919012)
(2.023590, 0.932770)
(2.442053, 0.940901)
(2.947052, 0.950594)
(3.556480, 0.961538)
(4.291934, 0.967167)
(5.179475, 0.973108)
(6.250552, 0.978111)
(7.543120, 0.982802)
(9.102982, 0.984991)
(10.985411, 0.988743)
(13.257114, 0.991557)
(15.998587, 0.995310)
(19.306977, 0.997498)
(23.299518, 0.998437)
(28.117687, 0.998749)
(33.932218, 0.999375)
(40.949151, 0.999375)
(49.417134, 0.999687)
(59.636233, 1.000000)
(71.968567, 1.000000)
(86.851137, 1.000000)
(104.811313, 1.000000)
(126.485522, 1.000000)
(152.641797, 1.000000)
(184.206997, 1.000000)
(222.299648, 1.000000)
(268.269580, 1.000000)
(323.745754, 1.000000)
(390.693994, 1.000000)
(471.486636, 1.000000)
(568.986603, 1.000000)
(686.648845, 1.000000)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer8_oampW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.000000)
(0.120679, 0.001254)
(0.145635, 0.003135)
(0.175751, 0.005956)
(0.212095, 0.010031)
(0.255955, 0.019749)
(0.308884, 0.035110)
(0.372759, 0.048276)
(0.449843, 0.067085)
(0.542868, 0.084639)
(0.655129, 0.100940)
(0.790604, 0.118495)
(0.954095, 0.138558)
(1.151395, 0.157994)
(1.389495, 0.179937)
(1.676833, 0.197492)
(2.023590, 0.214734)
(2.442053, 0.236677)
(2.947052, 0.254859)
(3.556480, 0.274608)
(4.291934, 0.291223)
(5.179475, 0.314420)
(6.250552, 0.334169)
(7.543120, 0.360502)
(9.102982, 0.378056)
(10.985411, 0.398433)
(13.257114, 0.423197)
(15.998587, 0.450470)
(19.306977, 0.475862)
(23.299518, 0.507210)
(28.117687, 0.534169)
(33.932218, 0.557680)
(40.949151, 0.584953)
(49.417134, 0.612853)
(59.636233, 0.643260)
(71.968567, 0.669592)
(86.851137, 0.689028)
(104.811313, 0.713793)
(126.485522, 0.730408)
(152.641797, 0.756740)
(184.206997, 0.782445)
(222.299648, 0.805016)
(268.269580, 0.833542)
(323.745754, 0.858621)
(390.693994, 0.884953)
(471.486636, 0.913793)
(568.986603, 0.946708)
(686.648845, 0.972100)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer9_learnW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.002815)
(0.120679, 0.015952)
(0.145635, 0.050985)
(0.175751, 0.105724)
(0.212095, 0.199249)
(0.255955, 0.314044)
(0.308884, 0.442915)
(0.372759, 0.569909)
(0.449843, 0.674695)
(0.542868, 0.747576)
(0.655129, 0.803253)
(0.790604, 0.847670)
(0.954095, 0.875821)
(1.151395, 0.898655)
(1.389495, 0.917110)
(1.676833, 0.929309)
(2.023590, 0.939944)
(2.442053, 0.950891)
(2.947052, 0.959337)
(3.556480, 0.967782)
(4.291934, 0.972787)
(5.179475, 0.977479)
(6.250552, 0.981545)
(7.543120, 0.985299)
(9.102982, 0.988739)
(10.985411, 0.991242)
(13.257114, 0.993431)
(15.998587, 0.995308)
(19.306977, 0.996246)
(23.299518, 0.996559)
(28.117687, 0.997185)
(33.932218, 0.997185)
(40.949151, 0.997810)
(49.417134, 0.999374)
(59.636233, 0.999687)
(71.968567, 1.000000)
(86.851137, 1.000000)
(104.811313, 1.000000)
(126.485522, 1.000000)
(152.641797, 1.000000)
(184.206997, 1.000000)
(222.299648, 1.000000)
(268.269580, 1.000000)
(323.745754, 1.000000)
(390.693994, 1.000000)
(471.486636, 1.000000)
(568.986603, 1.000000)
(686.648845, 1.000000)
(828.642773, 1.000000)
};

==> figures/rawfiles/anderson_score_cdf/hist_layer9_oampW.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(0.100000, 0.000000)
(0.120679, 0.001250)
(0.145635, 0.003125)
(0.175751, 0.007187)
(0.212095, 0.012500)
(0.255955, 0.023438)
(0.308884, 0.038125)
(0.372759, 0.055625)
(0.449843, 0.074375)
(0.542868, 0.091875)
(0.655129, 0.113437)
(0.790604, 0.136250)
(0.954095, 0.155000)
(1.151395, 0.180312)
(1.389495, 0.200937)
(1.676833, 0.220312)
(2.023590, 0.241250)
(2.442053, 0.260625)
(2.947052, 0.282812)
(3.556480, 0.301250)
(4.291934, 0.324062)
(5.179475, 0.352812)
(6.250552, 0.377187)
(7.543120, 0.409687)
(9.102982, 0.433437)
(10.985411, 0.464375)
(13.257114, 0.492500)
(15.998587, 0.524062)
(19.306977, 0.555312)
(23.299518, 0.585000)
(28.117687, 0.624375)
(33.932218, 0.657187)
(40.949151, 0.682812)
(49.417134, 0.710625)
(59.636233, 0.735000)
(71.968567, 0.756250)
(86.851137, 0.784062)
(104.811313, 0.807187)
(126.485522, 0.828750)
(152.641797, 0.854375)
(184.206997, 0.875938)
(222.299648, 0.894375)
(268.269580, 0.910625)
(323.745754, 0.933125)
(390.693994, 0.956875)
(471.486636, 0.966562)
(568.986603, 0.984062)
(686.648845, 0.999375)
(828.642773, 1.000000)
};

==> figures/rawfiles/andersonvscond/andersonvscond_learnW_0.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 0.421862)
(17.552568, 0.394342)
(18.638512, 0.323536)
(18.546717, 0.350766)
(13.428638, 0.409267)
(16.794140, 0.434243)
(14.297143, 0.327490)
(17.171722, 0.366975)
(20.059292, 0.440258)
(11.256145, 0.379654)
(25.958267, 0.315220)
(14.636854, 0.305723)
(16.587755, 0.349028)
(8.500388, 0.376624)
(19.118383, 0.449300)
(19.355614, 0.484575)
(16.919485, 0.300741)
(10.740816, 0.348816)
(24.433674, 0.385454)
(15.328254, 0.363767)
(15.667542, 0.347448)
(32.651962, 0.544521)
(14.833853, 0.360687)
(24.772644, 0.357145)
(19.206205, 0.362032)
(18.807907, 0.393727)
(20.472019, 0.405046)
(24.486319, 0.324483)
(13.134361, 0.343169)
(14.394195, 0.318407)
(16.070848, 0.345017)
(25.167027, 0.317807)
(15.581610, 0.381218)
(17.096106, 0.374512)
(21.280998, 0.398387)
(23.876585, 0.311603)
(13.036207, 0.365301)
(22.731215, 0.507054)
(35.325077, 0.423981)
(24.573538, 0.386436)
(22.238827, 0.390458)
(17.241997, 0.333399)
(21.504358, 0.344443)
(16.334728, 0.357794)
(18.660828, 0.456699)
(10.326597, 0.399092)
(16.468248, 0.348775)
(13.946894, 0.380204)
(33.479321, 0.372979)
(13.391328, 0.404579)
(16.313137, 0.382619)
(17.417023, 0.412869)
(14.955702, 0.357428)
(23.593338, 0.380474)
(25.343109, 0.436115)
(28.576508, 0.366524)
(26.743855, 0.467328)
(17.670483, 0.308095)
(14.859500, 0.368666)
(13.146446, 0.441910)
(16.851610, 0.422080)
(24.674076, 0.454631)
(14.513160, 0.345827)
(18.443485, 0.324835)
(13.139583, 0.314780)
(13.289401, 0.308966)
(13.496741, 0.406719)
(17.107384, 0.358376)
(9.916093, 0.325185)
(12.541000, 0.311617)
(13.952982, 0.348510)
(19.874964, 0.426205)
(36.316109, 0.544664)
(14.172893, 0.359938)
(8.225883, 0.327819)
(13.984437, 0.312090)
(32.250385, 0.422476)
(20.073103, 0.405990)
(18.860682, 0.441785)
(21.450701, 0.377394)
(12.890105, 0.350150)
(20.801798, 0.329354)
(20.644512, 0.339960)
(19.323544, 0.473400)
(12.121391, 0.342006)
(15.076665, 0.401439)
(15.545311, 0.421667)
(15.126464, 0.425699)
(8.966540, 0.347384)
(14.076862, 0.323442)
(18.888176, 0.461999)
(12.218390, 0.321090)
(27.091944, 0.446160)
(8.184272, 0.327147)
(21.078032, 0.403143)
(34.766178, 0.360208)
(24.455320, 0.382411)
(9.089629, 0.337549)
(18.335535, 0.343695)
(10.185403, 0.387690)
};


==> figures/rawfiles/andersonvscond/andersonvscond_learnW_1.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 1.345396)
(17.552568, 1.107674)
(18.638512, 0.956744)
(18.546717, 0.833950)
(13.428638, 1.682733)
(16.794140, 1.921507)
(14.297143, 0.937901)
(17.171722, 1.171004)
(20.059292, 1.339022)
(11.256145, 0.945443)
(25.958267, 1.355318)
(14.636854, 2.517780)
(16.587755, 0.848224)
(8.500388, 0.738479)
(19.118383, 1.212165)
(19.355614, 3.034812)
(16.919485, 1.207038)
(10.740816, 2.166728)
(24.433674, 0.766936)
(15.328254, 2.162299)
(15.667542, 1.755002)
(32.651962, 2.574189)
(14.833853, 1.304032)
(24.772644, 0.845651)
(19.206205, 1.910349)
(18.807907, 2.544941)
(20.472019, 1.415145)
(24.486319, 1.077110)
(13.134361, 1.920330)
(14.394195, 0.534307)
(16.070848, 2.209210)
(25.167027, 1.205170)
(15.581610, 3.080623)
(17.096106, 2.290631)
(21.280998, 0.646759)
(23.876585, 1.150585)
(13.036207, 2.457434)
(22.731215, 1.392491)
(35.325077, 0.760309)
(24.573538, 1.032725)
(22.238827, 2.385833)
(17.241997, 2.089184)
(21.504358, 0.755592)
(16.334728, 2.417822)
(18.660828, 2.015178)
(10.326597, 1.155728)
(16.468248, 2.720516)
(13.946894, 0.975270)
(33.479321, 0.623929)
(13.391328, 2.130270)
(16.313137, 1.792442)
(17.417023, 1.346748)
(14.955702, 4.828742)
(23.593338, 1.609913)
(25.343109, 1.415830)
(28.576508, 1.311487)
(26.743855, 1.449145)
(17.670483, 0.897684)
(14.859500, 3.091974)
(13.146446, 0.780744)
(16.851610, 1.265684)
(24.674076, 1.849046)
(14.513160, 1.474249)
(18.443485, 3.461485)
(13.139583, 2.612884)
(13.289401, 2.347485)
(13.496741, 0.820021)
(17.107384, 1.196670)
(9.916093, 1.212895)
(12.541000, 0.785657)
(13.952982, 0.704712)
(19.874964, 2.267964)
(36.316109, 0.490863)
(14.172893, 1.829737)
(8.225883, 1.369867)
(13.984437, 0.993298)
(32.250385, 0.887237)
(20.073103, 1.100760)
(18.860682, 1.462727)
(21.450701, 2.999602)
(12.890105, 0.988713)
(20.801798, 3.556688)
(20.644512, 0.951726)
(19.323544, 3.301617)
(12.121391, 1.149268)
(15.076665, 1.571449)
(15.545311, 2.099308)
(15.126464, 2.154840)
(8.966540, 0.782838)
(14.076862, 1.793021)
(18.888176, 1.734248)
(12.218390, 1.276617)
(27.091944, 2.135971)
(8.184272, 0.685841)
(21.078032, 0.869321)
(34.766178, 0.749110)
(24.455320, 1.247674)
(9.089629, 2.649663)
(18.335535, 2.963556)
(10.185403, 2.202037)
};


==> figures/rawfiles/andersonvscond/andersonvscond_learnW_2.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 0.442194)
(17.552568, 0.453690)
(18.638512, 0.790566)
(18.546717, 0.552865)
(13.428638, 0.672312)
(16.794140, 5.033959)
(14.297143, 0.437168)
(17.171722, 0.650743)
(20.059292, 2.583429)
(11.256145, 0.436920)
(25.958267, 1.596242)
(14.636854, 1.324226)
(16.587755, 0.505719)
(8.500388, 0.517311)
(19.118383, 0.785217)
(19.355614, 3.440516)
(16.919485, 0.788058)
(10.740816, 0.593079)
(24.433674, 1.415892)
(15.328254, 0.687175)
(15.667542, 0.490176)
(32.651962, 9.412439)
(14.833853, 0.443995)
(24.772644, 1.646902)
(19.206205, 0.769983)
(18.807907, 1.714580)
(20.472019, 0.941581)
(24.486319, 4.920434)
(13.134361, 0.568564)
(14.394195, 0.390517)
(16.070848, 0.671709)
(25.167027, 2.319960)
(15.581610, 0.522593)
(17.096106, 1.163661)
(21.280998, 1.027888)
(23.876585, 3.309568)
(13.036207, 0.498746)
(22.731215, 3.032594)
(35.325077, 3.204377)
(24.573538, 1.772425)
(22.238827, 1.294428)
(17.241997, 1.145256)
(21.504358, 2.133197)
(16.334728, 1.289152)
(18.660828, 1.142307)
(10.326597, 0.344365)
(16.468248, 0.979947)
(13.946894, 0.539008)
(33.479321, 3.727251)
(13.391328, 1.100087)
(16.313137, 0.885927)
(17.417023, 0.503588)
(14.955702, 2.526585)
(23.593338, 1.279559)
(25.343109, 1.933977)
(28.576508, 3.700497)
(26.743855, 4.572919)
(17.670483, 0.437166)
(14.859500, 2.053128)
(13.146446, 0.475842)
(16.851610, 0.547066)
(24.674076, 4.383716)
(14.513160, 0.429649)
(18.443485, 0.774302)
(13.139583, 0.714916)
(13.289401, 0.558458)
(13.496741, 0.356348)
(17.107384, 0.697882)
(9.916093, 0.371963)
(12.541000, 0.392886)
(13.952982, 0.491558)
(19.874964, 2.136024)
(36.316109, 4.232245)
(14.172893, 0.496567)
(8.225883, 0.385113)
(13.984437, 0.453461)
(32.250385, 3.638475)
(20.073103, 0.997361)
(18.860682, 0.982340)
(21.450701, 0.655337)
(12.890105, 0.549856)
(20.801798, 2.215275)
(20.644512, 0.985792)
(19.323544, 9.102635)
(12.121391, 0.663812)
(15.076665, 0.509300)
(15.545311, 2.978218)
(15.126464, 2.312412)
(8.966540, 0.382563)
(14.076862, 2.157771)
(18.888176, 2.883504)
(12.218390, 0.411146)
(27.091944, 5.592404)
(8.184272, 0.295129)
(21.078032, 0.951374)
(34.766178, 3.425006)
(24.455320, 1.563365)
(9.089629, 0.628394)
(18.335535, 1.307417)
(10.185403, 0.524986)
};


==> figures/rawfiles/andersonvscond/andersonvscond_learnW_3.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 0.422502)
(17.552568, 0.344041)
(18.638512, 0.444116)
(18.546717, 0.376385)
(13.428638, 0.459938)
(16.794140, 2.527487)
(14.297143, 0.374294)
(17.171722, 0.397294)
(20.059292, 1.293221)
(11.256145, 0.373287)
(25.958267, 1.085540)
(14.636854, 0.514530)
(16.587755, 0.427009)
(8.500388, 0.357604)
(19.118383, 0.426147)
(19.355614, 2.923855)
(16.919485, 0.440978)
(10.740816, 0.433227)
(24.433674, 0.778171)
(15.328254, 0.527577)
(15.667542, 0.401349)
(32.651962, 4.654369)
(14.833853, 0.414068)
(24.772644, 0.764537)
(19.206205, 0.573983)
(18.807907, 0.720762)
(20.472019, 0.514336)
(24.486319, 4.996832)
(13.134361, 0.386593)
(14.394195, 0.368693)
(16.070848, 0.365898)
(25.167027, 1.495251)
(15.581610, 0.393852)
(17.096106, 0.709826)
(21.280998, 0.542986)
(23.876585, 2.078959)
(13.036207, 0.365191)
(22.731215, 1.203706)
(35.325077, 5.823101)
(24.573538, 1.058083)
(22.238827, 1.346048)
(17.241997, 0.479202)
(21.504358, 1.550232)
(16.334728, 0.641979)
(18.660828, 0.745069)
(10.326597, 0.377314)
(16.468248, 0.555751)
(13.946894, 0.453794)
(33.479321, 2.166306)
(13.391328, 0.592974)
(16.313137, 0.560185)
(17.417023, 0.393126)
(14.955702, 1.038951)
(23.593338, 0.844366)
(25.343109, 4.266018)
(28.576508, 1.791477)
(26.743855, 2.683047)
(17.670483, 0.389380)
(14.859500, 0.741837)
(13.146446, 0.382212)
(16.851610, 0.500184)
(24.674076, 4.309954)
(14.513160, 0.482380)
(18.443485, 0.453145)
(13.139583, 0.392435)
(13.289401, 0.298451)
(13.496741, 0.346655)
(17.107384, 0.378505)
(9.916093, 0.345160)
(12.541000, 0.337258)
(13.952982, 0.341556)
(19.874964, 1.387728)
(36.316109, 14.893175)
(14.172893, 0.329399)
(8.225883, 0.337296)
(13.984437, 0.404677)
(32.250385, 4.128281)
(20.073103, 0.514999)
(18.860682, 0.683439)
(21.450701, 0.474865)
(12.890105, 0.423932)
(20.801798, 1.217175)
(20.644512, 0.543787)
(19.323544, 4.030807)
(12.121391, 0.384533)
(15.076665, 0.349569)
(15.545311, 1.169971)
(15.126464, 1.909299)
(8.966540, 0.352601)
(14.076862, 0.975553)
(18.888176, 0.827672)
(12.218390, 0.307499)
(27.091944, 4.232107)
(8.184272, 0.388749)
(21.078032, 0.597581)
(34.766178, 3.698667)
(24.455320, 0.895113)
(9.089629, 0.423106)
(18.335535, 0.483398)
(10.185403, 0.380847)
};


==> figures/rawfiles/andersonvscond/andersonvscond_learnW_4.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 0.318918)
(17.552568, 0.421654)
(18.638512, 0.372743)
(18.546717, 0.375568)
(13.428638, 0.368255)
(16.794140, 2.242649)
(14.297143, 0.372310)
(17.171722, 0.428842)
(20.059292, 0.976278)
(11.256145, 0.389019)
(25.958267, 0.592585)
(14.636854, 0.395521)
(16.587755, 0.328709)
(8.500388, 0.342165)
(19.118383, 0.342490)
(19.355614, 2.144680)
(16.919485, 0.367664)
(10.740816, 0.401085)
(24.433674, 0.422234)
(15.328254, 0.330045)
(15.667542, 0.404764)
(32.651962, 3.605156)
(14.833853, 0.406017)
(24.772644, 0.567241)
(19.206205, 0.420952)
(18.807907, 0.570500)
(20.472019, 0.478749)
(24.486319, 3.902798)
(13.134361, 0.395544)
(14.394195, 0.350427)
(16.070848, 0.391106)
(25.167027, 1.075280)
(15.581610, 0.389157)
(17.096106, 0.511522)
(21.280998, 0.434627)
(23.876585, 0.755710)
(13.036207, 0.310945)
(22.731215, 0.771127)
(35.325077, 2.761506)
(24.573538, 0.775508)
(22.238827, 0.743653)
(17.241997, 0.369942)
(21.504358, 1.605489)
(16.334728, 0.476571)
(18.660828, 0.471833)
(10.326597, 0.271068)
(16.468248, 0.448655)
(13.946894, 0.387286)
(33.479321, 2.218845)
(13.391328, 0.600067)
(16.313137, 0.417739)
(17.417023, 0.393832)
(14.955702, 0.625995)
(23.593338, 0.783570)
(25.343109, 2.386741)
(28.576508, 1.400046)
(26.743855, 1.279856)
(17.670483, 0.358924)
(14.859500, 0.619143)
(13.146446, 0.448645)
(16.851610, 0.526081)
(24.674076, 3.495887)
(14.513160, 0.368754)
(18.443485, 0.410358)
(13.139583, 0.400848)
(13.289401, 0.356789)
(13.496741, 0.323740)
(17.107384, 0.413238)
(9.916093, 0.343007)
(12.541000, 0.355713)
(13.952982, 0.317422)
(19.874964, 1.214827)
(36.316109, 9.256732)
(14.172893, 0.372669)
(8.225883, 0.373296)
(13.984437, 0.416039)
(32.250385, 4.229172)
(20.073103, 0.414695)
(18.860682, 0.516063)
(21.450701, 0.383745)
(12.890105, 0.459385)
(20.801798, 0.758129)
(20.644512, 0.442369)
(19.323544, 1.380759)
(12.121391, 0.326456)
(15.076665, 0.318396)
(15.545311, 0.636719)
(15.126464, 0.922065)
(8.966540, 0.342766)
(14.076862, 0.707698)
(18.888176, 0.621426)
(12.218390, 0.327408)
(27.091944, 4.319929)
(8.184272, 0.307267)
(21.078032, 0.419516)
(34.766178, 1.620056)
(24.455320, 0.605857)
(9.089629, 0.397571)
(18.335535, 0.549249)
(10.185403, 0.336104)
};


==> figures/rawfiles/andersonvscond/andersonvscond_learnW_5.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(26.244871, 0.377897)
(17.552568, 0.291790)
(18.638512, 0.346613)
(18.546717, 0.330534)
(13.428638, 0.301845)
(16.794140, 1.684237)
(14.297143, 0.338368)
(17.171722, 0.360197)
(20.059292, 0.873285)
(11.256145, 0.298155)
(25.958267, 0.807828)
(14.636854, 0.390494)
(16.587755, 0.364455)
(8.500388, 0.396100)
(19.118383, 0.447113)
(19.355614, 0.857754)
(16.919485, 0.352021)
(10.740816, 0.418349)
(24.433674, 0.406303)
(15.328254, 0.308162)
(15.667542, 0.349054)
(32.651962, 2.613025)
(14.833853, 0.340947)
(24.772644, 0.527418)
(19.206205, 0.511693)
(18.807907, 0.588920)
(20.472019, 0.374495)
(24.486319, 2.344508)
(13.134361, 0.396579)
(14.394195, 0.377126)
(16.070848, 0.437433)
(25.167027, 0.766479)
(15.581610, 0.371293)
(17.096106, 0.437601)
(21.280998, 0.373360)
(23.876585, 0.511140)
(13.036207, 0.410883)
(22.731215, 0.815002)
(35.325077, 2.312334)
(24.573538, 0.674081)
(22.238827, 0.734588)
(17.241997, 0.392292)
(21.504358, 1.051083)
(16.334728, 0.500520)
(18.660828, 0.494484)
(10.326597, 0.285771)
(16.468248, 0.406523)
(13.946894, 0.346071)
(33.479321, 1.381222)
(13.391328, 0.421834)
(16.313137, 0.412466)
(17.417023, 0.395421)
(14.955702, 0.557012)
(23.593338, 0.798257)
(25.343109, 2.176534)
(28.576508, 0.797968)
(26.743855, 1.205859)
(17.670483, 0.362377)
(14.859500, 0.509730)
(13.146446, 0.404986)
(16.851610, 0.427092)
(24.674076, 2.597760)
(14.513160, 0.275339)
(18.443485, 0.416281)
(13.139583, 0.348166)
(13.289401, 0.297446)
(13.496741, 0.269053)
(17.107384, 0.379414)
(9.916093, 0.300410)
(12.541000, 0.332992)
(13.952982, 0.320399)
(19.874964, 0.999565)
(36.316109, 9.506243)
(14.172893, 0.473200)
(8.225883, 0.369551)
(13.984437, 0.390900)
(32.250385, 3.221076)
(20.073103, 0.455855)
(18.860682, 0.628496)
(21.450701, 0.334832)
(12.890105, 0.407406)
(20.801798, 0.831442)
(20.644512, 0.371411)
(19.323544, 1.477988)
(12.121391, 0.373209)
(15.076665, 0.303889)
(15.545311, 0.503972)
(15.126464, 0.688844)
(8.966540, 0.309568)
(14.076862, 0.893872)
(18.888176, 0.649390)
(12.218390, 0.300266)
(27.091944, 2.965926)
(8.184272, 0.329591)
(21.078032, 0.361148)
(34.766178, 2.021144)
(24.455320, 0.583449)
(9.089629, 0.339088)
(18.335535, 0.504839)
(10.185403, 0.371931)
};


==> figures/rawfiles/andersonvscond/andersonvscond_learnW_6.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(26.244871, 0.368323)
(17.552568, 0.349237)
(18.638512, 0.341879)
(18.546717, 0.338001)
(13.428638, 0.355754)
(16.794140, 1.681132)
(14.297143, 0.405086)
(17.171722, 0.299309)
(20.059292, 0.589026)
(11.256145, 0.324177)
(25.958267, 0.790381)
(14.636854, 0.292965)
(16.587755, 0.333433)
(8.500388, 0.455507)
(19.118383, 0.339585)
(19.355614, 1.040454)
(16.919485, 0.371759)
(10.740816, 0.382154)
(24.433674, 0.356676)
(15.328254, 0.381578)
(15.667542, 0.388126)
(32.651962, 2.478085)
(14.833853, 0.373369)
(24.772644, 0.446930)
(19.206205, 0.343719)
(18.807907, 0.434640)
(20.472019, 0.379036)
(24.486319, 1.926467)
(13.134361, 0.379297)
(14.394195, 0.273402)
(16.070848, 0.433087)
(25.167027, 0.687977)
(15.581610, 0.308742)
(17.096106, 0.368579)
(21.280998, 0.369643)
(23.876585, 0.478515)
(13.036207, 0.330998)
(22.731215, 0.749134)
(35.325077, 2.250507)
(24.573538, 0.595435)
(22.238827, 0.470244)
(17.241997, 0.393993)
(21.504358, 0.849114)
(16.334728, 0.437228)
(18.660828, 0.525934)
(10.326597, 0.349085)
(16.468248, 0.360759)
(13.946894, 0.385318)
(33.479321, 1.194840)
(13.391328, 0.389860)
(16.313137, 0.373932)
(17.417023, 0.372871)
(14.955702, 0.437743)
(23.593338, 0.673427)
(25.343109, 1.356016)
(28.576508, 1.058840)
(26.743855, 0.973275)
(17.670483, 0.353693)
(14.859500, 0.430808)
(13.146446, 0.422799)
(16.851610, 0.419200)
(24.674076, 1.323633)
(14.513160, 0.322233)
(18.443485, 0.406237)
(13.139583, 0.346306)
(13.289401, 0.256231)
(13.496741, 0.317552)
(17.107384, 0.360463)
(9.916093, 0.327037)
(12.541000, 0.329074)
(13.952982, 0.334940)
(19.874964, 0.623802)
(36.316109, 7.592923)
(14.172893, 0.295631)
(8.225883, 0.389184)
(13.984437, 0.332786)
(32.250385, 2.892167)
(20.073103, 0.369700)
(18.860682, 0.595617)
(21.450701, 0.359697)
(12.890105, 0.367761)
(20.801798, 0.641646)
(20.644512, 0.430736)
(19.323544, 1.065751)
(12.121391, 0.349126)
(15.076665, 0.344912)
(15.545311, 0.425201)
(15.126464, 0.460353)
(8.966540, 0.349606)
(14.076862, 0.896430)
(18.888176, 0.602454)
(12.218390, 0.306147)
(27.091944, 5.245297)
(8.184272, 0.370288)
(21.078032, 0.354597)
(34.766178, 1.860713)
(24.455320, 0.623805)
(9.089629, 0.359320)
(18.335535, 0.488869)
(10.185403, 0.392265)
};


==> figures/rawfiles/andersonvscond/andersonvscond_learnW_7.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(26.244871, 0.326526)
(17.552568, 0.371191)
(18.638512, 0.339872)
(18.546717, 0.280481)
(13.428638, 0.387329)
(16.794140, 1.383480)
(14.297143, 0.351105)
(17.171722, 0.349941)
(20.059292, 0.574955)
(11.256145, 0.360021)
(25.958267, 0.713766)
(14.636854, 0.380494)
(16.587755, 0.359667)
(8.500388, 0.340420)
(19.118383, 0.423427)
(19.355614, 0.842083)
(16.919485, 0.327065)
(10.740816, 0.434058)
(24.433674, 0.373898)
(15.328254, 0.350893)
(15.667542, 0.407625)
(32.651962, 1.621581)
(14.833853, 0.366753)
(24.772644, 0.397664)
(19.206205, 0.332536)
(18.807907, 0.504089)
(20.472019, 0.380442)
(24.486319, 1.335394)
(13.134361, 0.386940)
(14.394195, 0.357952)
(16.070848, 0.345817)
(25.167027, 0.634196)
(15.581610, 0.379784)
(17.096106, 0.437373)
(21.280998, 0.392900)
(23.876585, 0.470582)
(13.036207, 0.364304)
(22.731215, 0.608597)
(35.325077, 1.935069)
(24.573538, 0.717825)
(22.238827, 0.451770)
(17.241997, 0.338745)
(21.504358, 0.763819)
(16.334728, 0.426797)
(18.660828, 0.456191)
(10.326597, 0.336048)
(16.468248, 0.318197)
(13.946894, 0.352733)
(33.479321, 1.107620)
(13.391328, 0.465058)
(16.313137, 0.358733)
(17.417023, 0.353484)
(14.955702, 0.434014)
(23.593338, 0.618944)
(25.343109, 1.116197)
(28.576508, 0.856655)
(26.743855, 0.962618)
(17.670483, 0.372803)
(14.859500, 0.473865)
(13.146446, 0.497510)
(16.851610, 0.370594)
(24.674076, 2.140121)
(14.513160, 0.351013)
(18.443485, 0.388312)
(13.139583, 0.348796)
(13.289401, 0.316990)
(13.496741, 0.285201)
(17.107384, 0.432174)
(9.916093, 0.284937)
(12.541000, 0.323739)
(13.952982, 0.304591)
(19.874964, 0.833493)
(36.316109, 8.005581)
(14.172893, 0.406849)
(8.225883, 0.336384)
(13.984437, 0.400335)
(32.250385, 2.374633)
(20.073103, 0.406411)
(18.860682, 0.524688)
(21.450701, 0.393669)
(12.890105, 0.377017)
(20.801798, 0.826570)
(20.644512, 0.389144)
(19.323544, 1.074502)
(12.121391, 0.370215)
(15.076665, 0.345462)
(15.545311, 0.410630)
(15.126464, 0.558019)
(8.966540, 0.410897)
(14.076862, 0.733799)
(18.888176, 0.496163)
(12.218390, 0.362372)
(27.091944, 3.448707)
(8.184272, 0.317596)
(21.078032, 0.340029)
(34.766178, 2.096818)
(24.455320, 0.418568)
(9.089629, 0.414479)
(18.335535, 0.426652)
(10.185403, 0.350836)
};


==> figures/rawfiles/andersonvscond/andersonvscond_learnW_8.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(26.244871, 0.336965)
(17.552568, 0.378631)
(18.638512, 0.322746)
(18.546717, 0.307167)
(13.428638, 0.301555)
(16.794140, 1.819173)
(14.297143, 0.362590)
(17.171722, 0.355598)
(20.059292, 0.565031)
(11.256145, 0.369155)
(25.958267, 0.854375)
(14.636854, 0.337253)
(16.587755, 0.373686)
(8.500388, 0.379922)
(19.118383, 0.286075)
(19.355614, 0.764356)
(16.919485, 0.399528)
(10.740816, 0.382582)
(24.433674, 0.359808)
(15.328254, 0.309780)
(15.667542, 0.337937)
(32.651962, 2.277350)
(14.833853, 0.361256)
(24.772644, 0.374608)
(19.206205, 0.382559)
(18.807907, 0.468039)
(20.472019, 0.319001)
(24.486319, 1.195746)
(13.134361, 0.399963)
(14.394195, 0.307414)
(16.070848, 0.351748)
(25.167027, 0.495715)
(15.581610, 0.333019)
(17.096106, 0.418151)
(21.280998, 0.349883)
(23.876585, 0.549684)
(13.036207, 0.351797)
(22.731215, 0.630025)
(35.325077, 1.489690)
(24.573538, 0.456154)
(22.238827, 0.407310)
(17.241997, 0.378582)
(21.504358, 0.747121)
(16.334728, 0.373674)
(18.660828, 0.454760)
(10.326597, 0.331787)
(16.468248, 0.345581)
(13.946894, 0.346796)
(33.479321, 0.846844)
(13.391328, 0.397394)
(16.313137, 0.454486)
(17.417023, 0.417879)
(14.955702, 0.429880)
(23.593338, 0.679727)
(25.343109, 1.183805)
(28.576508, 0.882393)
(26.743855, 0.837535)
(17.670483, 0.343258)
(14.859500, 0.495416)
(13.146446, 0.464222)
(16.851610, 0.430065)
(24.674076, 1.310387)
(14.513160, 0.393948)
(18.443485, 0.287192)
(13.139583, 0.399224)
(13.289401, 0.323260)
(13.496741, 0.321856)
(17.107384, 0.463561)
(9.916093, 0.297487)
(12.541000, 0.362514)
(13.952982, 0.346545)
(19.874964, 0.581645)
(36.316109, 4.513060)
(14.172893, 0.360181)
(8.225883, 0.412439)
(13.984437, 0.368198)
(32.250385, 1.907233)
(20.073103, 0.354904)
(18.860682, 0.482435)
(21.450701, 0.381205)
(12.890105, 0.407182)
(20.801798, 0.548985)
(20.644512, 0.449479)
(19.323544, 0.759416)
(12.121391, 0.411234)
(15.076665, 0.301975)
(15.545311, 0.429653)
(15.126464, 0.483522)
(8.966540, 0.337918)
(14.076862, 0.797912)
(18.888176, 0.511858)
(12.218390, 0.345471)
(27.091944, 3.767615)
(8.184272, 0.351148)
(21.078032, 0.389638)
(34.766178, 1.300675)
(24.455320, 0.449754)
(9.089629, 0.342966)
(18.335535, 0.443143)
(10.185403, 0.377234)
};


==> figures/rawfiles/andersonvscond/andersonvscond_learnW_9.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(26.244871, 0.335423)
(17.552568, 0.340977)
(18.638512, 0.301659)
(18.546717, 0.385651)
(13.428638, 0.378178)
(16.794140, 1.080431)
(14.297143, 0.281820)
(17.171722, 0.319892)
(20.059292, 0.490438)
(11.256145, 0.396085)
(25.958267, 0.520594)
(14.636854, 0.366384)
(16.587755, 0.362477)
(8.500388, 0.313245)
(19.118383, 0.370261)
(19.355614, 0.748834)
(16.919485, 0.371489)
(10.740816, 0.390886)
(24.433674, 0.425545)
(15.328254, 0.305550)
(15.667542, 0.395800)
(32.651962, 1.352403)
(14.833853, 0.329894)
(24.772644, 0.342578)
(19.206205, 0.345538)
(18.807907, 0.425313)
(20.472019, 0.298506)
(24.486319, 0.965094)
(13.134361, 0.361319)
(14.394195, 0.318976)
(16.070848, 0.360450)
(25.167027, 0.481192)
(15.581610, 0.346252)
(17.096106, 0.390772)
(21.280998, 0.401717)
(23.876585, 0.429211)
(13.036207, 0.336386)
(22.731215, 0.695010)
(35.325077, 0.968110)
(24.573538, 0.495852)
(22.238827, 0.496976)
(17.241997, 0.363560)
(21.504358, 0.643956)
(16.334728, 0.330605)
(18.660828, 0.464704)
(10.326597, 0.376247)
(16.468248, 0.382290)
(13.946894, 0.352263)
(33.479321, 0.617898)
(13.391328, 0.428018)
(16.313137, 0.319986)
(17.417023, 0.370851)
(14.955702, 0.370919)
(23.593338, 0.564751)
(25.343109, 0.893050)
(28.576508, 0.830187)
(26.743855, 0.823112)
(17.670483, 0.349827)
(14.859500, 0.439585)
(13.146446, 0.330085)
(16.851610, 0.401028)
(24.674076, 1.257695)
(14.513160, 0.371345)
(18.443485, 0.364113)
(13.139583, 0.329159)
(13.289401, 0.295353)
(13.496741, 0.348457)
(17.107384, 0.436098)
(9.916093, 0.349136)
(12.541000, 0.305671)
(13.952982, 0.354689)
(19.874964, 0.567336)
(36.316109, 3.663760)
(14.172893, 0.404986)
(8.225883, 0.304306)
(13.984437, 0.358660)
(32.250385, 1.443004)
(20.073103, 0.309177)
(18.860682, 0.550687)
(21.450701, 0.349771)
(12.890105, 0.362198)
(20.801798, 0.641778)
(20.644512, 0.396349)
(19.323544, 0.883000)
(12.121391, 0.378854)
(15.076665, 0.362135)
(15.545311, 0.373218)
(15.126464, 0.462445)
(8.966540, 0.290476)
(14.076862, 0.923650)
(18.888176, 0.428395)
(12.218390, 0.318876)
(27.091944, 2.314496)
(8.184272, 0.280567)
(21.078032, 0.381628)
(34.766178, 1.218385)
(24.455320, 0.414574)
(9.089629, 0.386516)
(18.335535, 0.467409)
(10.185403, 0.345818)
};


==> figures/rawfiles/andersonvscond/andersonvscond_oampW_0.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 0.379840)
(17.552568, 0.286021)
(18.638512, 0.338603)
(18.546717, 0.314787)
(13.428638, 0.368547)
(16.794140, 0.413787)
(14.297143, 0.343933)
(17.171722, 0.465583)
(20.059292, 0.403804)
(11.256145, 0.458252)
(25.958267, 0.318423)
(14.636854, 0.369417)
(16.587755, 0.404538)
(8.500388, 0.392059)
(19.118383, 0.430447)
(19.355614, 0.454362)
(16.919485, 0.322738)
(10.740816, 0.356044)
(24.433674, 0.414281)
(15.328254, 0.384003)
(15.667542, 0.475693)
(32.651962, 0.359253)
(14.833853, 0.375851)
(24.772644, 0.447000)
(19.206205, 0.344703)
(18.807907, 0.463462)
(20.472019, 0.425012)
(24.486319, 0.386715)
(13.134361, 0.329982)
(14.394195, 0.444701)
(16.070848, 0.328187)
(25.167027, 0.390681)
(15.581610, 0.438790)
(17.096106, 0.447989)
(21.280998, 0.340984)
(23.876585, 0.321970)
(13.036207, 0.323143)
(22.731215, 0.391188)
(35.325077, 0.378518)
(24.573538, 0.425728)
(22.238827, 0.522920)
(17.241997, 0.361205)
(21.504358, 0.427659)
(16.334728, 0.387778)
(18.660828, 0.421342)
(10.326597, 0.407889)
(16.468248, 0.366819)
(13.946894, 0.342912)
(33.479321, 0.583428)
(13.391328, 0.340577)
(16.313137, 0.621129)
(17.417023, 0.295969)
(14.955702, 0.449104)
(23.593338, 0.485342)
(25.343109, 0.329479)
(28.576508, 0.396631)
(26.743855, 0.340560)
(17.670483, 0.399894)
(14.859500, 0.313221)
(13.146446, 0.403187)
(16.851610, 0.375396)
(24.674076, 0.389058)
(14.513160, 0.404665)
(18.443485, 0.435022)
(13.139583, 0.373012)
(13.289401, 0.466090)
(13.496741, 0.705708)
(17.107384, 0.389442)
(9.916093, 0.308432)
(12.541000, 0.355770)
(13.952982, 0.379636)
(19.874964, 0.364288)
(36.316109, 0.438612)
(14.172893, 0.306868)
(8.225883, 0.442266)
(13.984437, 0.313547)
(32.250385, 0.463853)
(20.073103, 0.488316)
(18.860682, 0.415150)
(21.450701, 0.403990)
(12.890105, 0.360824)
(20.801798, 0.397800)
(20.644512, 0.330134)
(19.323544, 0.441926)
(12.121391, 0.350884)
(15.076665, 0.331571)
(15.545311, 0.352627)
(15.126464, 0.356930)
(8.966540, 0.405024)
(14.076862, 0.292299)
(18.888176, 0.434055)
(12.218390, 0.292334)
(27.091944, 0.360800)
(8.184272, 0.322949)
(21.078032, 0.330995)
(34.766178, 0.447153)
(24.455320, 0.561676)
(9.089629, 0.411008)
(18.335535, 0.388135)
(10.185403, 0.403464)
};


==> figures/rawfiles/andersonvscond/andersonvscond_oampW_1.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 14.660919)
(17.552568, 13.443987)
(18.638512, 14.988220)
(18.546717, 6.465210)
(13.428638, 18.012192)
(16.794140, 30.749175)
(14.297143, 15.365552)
(17.171722, 14.132895)
(20.059292, 12.373714)
(11.256145, 6.370485)
(25.958267, 7.612961)
(14.636854, 22.398839)
(16.587755, 12.395732)
(8.500388, 4.879955)
(19.118383, 10.588386)
(19.355614, 18.002642)
(16.919485, 15.771610)
(10.740816, 11.040487)
(24.433674, 5.920507)
(15.328254, 37.037491)
(15.667542, 30.227484)
(32.651962, 14.274474)
(14.833853, 19.979874)
(24.772644, 4.130780)
(19.206205, 48.235806)
(18.807907, 27.076395)
(20.472019, 8.170365)
(24.486319, 5.241664)
(13.134361, 26.020278)
(14.394195, 8.213191)
(16.070848, 30.087846)
(25.167027, 11.774505)
(15.581610, 27.397577)
(17.096106, 23.387734)
(21.280998, 4.390373)
(23.876585, 8.347487)
(13.036207, 22.938183)
(22.731215, 19.716553)
(35.325077, 3.660134)
(24.573538, 5.032256)
(22.238827, 17.821594)
(17.241997, 17.416712)
(21.504358, 2.033799)
(16.334728, 46.597145)
(18.660828, 34.308000)
(10.326597, 4.207761)
(16.468248, 26.248115)
(13.946894, 9.825288)
(33.479321, 0.971241)
(13.391328, 17.247865)
(16.313137, 20.818144)
(17.417023, 33.399826)
(14.955702, 41.548195)
(23.593338, 32.036667)
(25.343109, 22.940156)
(28.576508, 6.893595)
(26.743855, 19.182318)
(17.670483, 9.570843)
(14.859500, 36.041592)
(13.146446, 17.600180)
(16.851610, 28.130656)
(24.674076, 10.621376)
(14.513160, 21.423051)
(18.443485, 42.686459)
(13.139583, 18.701633)
(13.289401, 17.481078)
(13.496741, 15.984431)
(17.107384, 16.779113)
(9.916093, 2.297429)
(12.541000, 8.001464)
(13.952982, 22.891620)
(19.874964, 30.852823)
(36.316109, 1.342568)
(14.172893, 30.450837)
(8.225883, 1.723038)
(13.984437, 30.516502)
(32.250385, 2.084019)
(20.073103, 8.178579)
(18.860682, 29.527988)
(21.450701, 28.047029)
(12.890105, 13.669309)
(20.801798, 25.052029)
(20.644512, 18.720149)
(19.323544, 16.864935)
(12.121391, 18.320148)
(15.076665, 23.104898)
(15.545311, 18.395344)
(15.126464, 55.963593)
(8.966540, 2.764908)
(14.076862, 35.152607)
(18.888176, 23.213128)
(12.218390, 17.940981)
(27.091944, 7.277732)
(8.184272, 1.774066)
(21.078032, 13.120691)
(34.766178, 2.083123)
(24.455320, 2.153099)
(9.089629, 2.402379)
(18.335535, 35.207216)
(10.185403, 9.217000)
};


==> figures/rawfiles/andersonvscond/andersonvscond_oampW_2.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 15.914807)
(17.552568, 19.233951)
(18.638512, 30.615129)
(18.546717, 17.735394)
(13.428638, 5.560703)
(16.794140, 49.900245)
(14.297143, 3.415236)
(17.171722, 21.480158)
(20.059292, 57.277637)
(11.256145, 1.608307)
(25.958267, 71.092750)
(14.636854, 30.505452)
(16.587755, 3.808093)
(8.500388, 1.661200)
(19.118383, 31.604247)
(19.355614, 80.874956)
(16.919485, 19.551703)
(10.740816, 1.681509)
(24.433674, 37.679976)
(15.328254, 17.879289)
(15.667542, 20.041192)
(32.651962, 84.728378)
(14.833853, 8.997947)
(24.772644, 29.107440)
(19.206205, 69.980867)
(18.807907, 61.139298)
(20.472019, 26.375820)
(24.486319, 60.713939)
(13.134361, 7.037496)
(14.394195, 2.799932)
(16.070848, 23.737459)
(25.167027, 70.394957)
(15.581610, 14.352829)
(17.096106, 24.037571)
(21.280998, 33.754820)
(23.876585, 60.578868)
(13.036207, 8.237970)
(22.731215, 54.952111)
(35.325077, 84.211606)
(24.573538, 27.021661)
(22.238827, 116.899107)
(17.241997, 42.054457)
(21.504358, 28.881261)
(16.334728, 46.553673)
(18.660828, 38.841759)
(10.326597, 0.543500)
(16.468248, 25.256357)
(13.946894, 7.420597)
(33.479321, 32.559891)
(13.391328, 19.710273)
(16.313137, 38.916125)
(17.417023, 31.150837)
(14.955702, 40.712500)
(23.593338, 58.880677)
(25.343109, 97.731257)
(28.576508, 82.026081)
(26.743855, 66.502478)
(17.670483, 15.824713)
(14.859500, 55.295392)
(13.146446, 33.581422)
(16.851610, 21.156646)
(24.674076, 70.575042)
(14.513160, 15.189844)
(18.443485, 28.794304)
(13.139583, 13.005156)
(13.289401, 3.860343)
(13.496741, 3.738218)
(17.107384, 9.271707)
(9.916093, 0.839535)
(12.541000, 4.970075)
(13.952982, 7.907936)
(19.874964, 93.121082)
(36.316109, 29.347486)
(14.172893, 9.549923)
(8.225883, 0.572789)
(13.984437, 27.900621)
(32.250385, 49.505147)
(20.073103, 29.938075)
(18.860682, 62.758262)
(21.450701, 61.363304)
(12.890105, 6.586501)
(20.801798, 59.848100)
(20.644512, 42.159292)
(19.323544, 36.161626)
(12.121391, 16.662003)
(15.076665, 8.470577)
(15.545311, 23.239974)
(15.126464, 75.249826)
(8.966540, 0.884750)
(14.076862, 43.521248)
(18.888176, 91.113148)
(12.218390, 7.796780)
(27.091944, 49.297644)
(8.184272, 0.672939)
(21.078032, 17.974186)
(34.766178, 60.510083)
(24.455320, 48.754210)
(9.089629, 0.651543)
(18.335535, 78.151832)
(10.185403, 1.687631)
};


==> figures/rawfiles/andersonvscond/andersonvscond_oampW_3.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 15.361890)
(17.552568, 19.031446)
(18.638512, 26.587759)
(18.546717, 21.756800)
(13.428638, 2.646001)
(16.794140, 42.886868)
(14.297143, 1.956418)
(17.171722, 21.459686)
(20.059292, 63.375236)
(11.256145, 1.593092)
(25.958267, 82.337695)
(14.636854, 24.455186)
(16.587755, 3.149124)
(8.500388, 1.388191)
(19.118383, 36.047575)
(19.355614, 88.587367)
(16.919485, 10.671642)
(10.740816, 1.095561)
(24.433674, 42.629005)
(15.328254, 14.390462)
(15.667542, 18.659051)
(32.651962, 108.422587)
(14.833853, 6.962036)
(24.772644, 40.445722)
(19.206205, 61.837047)
(18.807907, 52.217957)
(20.472019, 29.639151)
(24.486319, 71.188139)
(13.134361, 6.706162)
(14.394195, 2.436094)
(16.070848, 13.850370)
(25.167027, 78.075547)
(15.581610, 10.860724)
(17.096106, 17.002390)
(21.280998, 47.129133)
(23.876585, 58.695450)
(13.036207, 5.656244)
(22.731215, 62.959732)
(35.325077, 117.036130)
(24.573538, 36.247918)
(22.238827, 121.707271)
(17.241997, 46.187085)
(21.504358, 30.013734)
(16.334728, 30.654390)
(18.660828, 34.576238)
(10.326597, 0.502623)
(16.468248, 13.420940)
(13.946894, 6.815807)
(33.479321, 63.928615)
(13.391328, 13.042007)
(16.313137, 39.050145)
(17.417023, 27.416648)
(14.955702, 22.430100)
(23.593338, 49.031925)
(25.343109, 120.184195)
(28.576508, 121.796152)
(26.743855, 96.176711)
(17.670483, 10.080786)
(14.859500, 46.012774)
(13.146446, 28.225678)
(16.851610, 14.481592)
(24.674076, 79.365693)
(14.513160, 15.904348)
(18.443485, 20.892037)
(13.139583, 7.593108)
(13.289401, 3.016108)
(13.496741, 2.811125)
(17.107384, 4.998537)
(9.916093, 0.664409)
(12.541000, 3.771991)
(13.952982, 7.206872)
(19.874964, 103.622849)
(36.316109, 81.470112)
(14.172893, 5.225656)
(8.225883, 0.576562)
(13.984437, 21.678090)
(32.250385, 66.622301)
(20.073103, 25.167883)
(18.860682, 50.846821)
(21.450701, 49.963449)
(12.890105, 6.202348)
(20.801798, 52.655403)
(20.644512, 42.562268)
(19.323544, 45.159053)
(12.121391, 14.465319)
(15.076665, 6.089660)
(15.545311, 21.976419)
(15.126464, 82.982074)
(8.966540, 0.845502)
(14.076862, 31.451422)
(18.888176, 92.516863)
(12.218390, 6.312876)
(27.091944, 64.359836)
(8.184272, 0.649116)
(21.078032, 18.505951)
(34.766178, 112.675711)
(24.455320, 80.196437)
(9.089629, 0.655810)
(18.335535, 89.256083)
(10.185403, 1.208279)
};


==> figures/rawfiles/andersonvscond/andersonvscond_oampW_4.tex <==
\addplot+ [only marks] coordinates{ 
(26.244871, 15.118831)
(17.552568, 18.901883)
(18.638512, 20.983134)
(18.546717, 14.985687)
(13.428638, 2.232663)
(16.794140, 39.762665)
(14.297143, 1.036462)
(17.171722, 20.741449)
(20.059292, 52.167524)
(11.256145, 1.359087)
(25.958267, 71.504787)
(14.636854, 21.388017)
(16.587755, 2.721594)
(8.500388, 1.249495)
(19.118383, 29.617399)
(19.355614, 94.433028)
(16.919485, 8.673978)
(10.740816, 0.986396)
(24.433674, 40.779976)
(15.328254, 7.447432)
(15.667542, 12.078360)
(32.651962, 119.632509)
(14.833853, 4.841748)
(24.772644, 35.985266)
(19.206205, 54.807661)
(18.807907, 41.751352)
(20.472019, 24.191299)
(24.486319, 68.277518)
(13.134361, 3.047329)
(14.394195, 2.183786)
(16.070848, 6.601949)
(25.167027, 54.317807)
(15.581610, 8.296091)
(17.096106, 19.603837)
(21.280998, 31.645542)
(23.876585, 45.099107)
(13.036207, 5.209524)
(22.731215, 58.398763)
(35.325077, 132.484750)
(24.573538, 32.245403)
(22.238827, 142.391577)
(17.241997, 38.974995)
(21.504358, 29.157986)
(16.334728, 26.857975)
(18.660828, 34.466062)
(10.326597, 0.490058)
(16.468248, 16.841907)
(13.946894, 6.874589)
(33.479321, 94.876957)
(13.391328, 9.133256)
(16.313137, 27.230056)
(17.417023, 28.707759)
(14.955702, 15.796970)
(23.593338, 37.423524)
(25.343109, 132.066446)
(28.576508, 106.874598)
(26.743855, 83.592924)
(17.670483, 6.169960)
(14.859500, 30.570173)
(13.146446, 13.265075)
(16.851610, 10.975506)
(24.674076, 85.859536)
(14.513160, 12.756195)
(18.443485, 20.009423)
(13.139583, 4.034076)
(13.289401, 2.098604)
(13.496741, 2.256473)
(17.107384, 2.810336)
(9.916093, 0.664647)
(12.541000, 3.580335)
(13.952982, 6.769436)
(19.874964, 104.163603)
(36.316109, 124.171015)
(14.172893, 3.956727)
(8.225883, 0.581463)
(13.984437, 16.144770)
(32.250385, 70.248625)
(20.073103, 20.429441)
(18.860682, 45.674943)
(21.450701, 42.483137)
(12.890105, 6.203615)
(20.801798, 42.365924)
(20.644512, 39.190654)
(19.323544, 39.617186)
(12.121391, 15.891299)
(15.076665, 4.790517)
(15.545311, 18.234509)
(15.126464, 68.870599)
(8.966540, 0.828546)
(14.076862, 23.168413)
(18.888176, 96.324247)
(12.218390, 4.896355)
(27.091944, 58.482841)
(8.184272, 0.551955)
(21.078032, 19.019530)
(34.766178, 130.278648)
(24.455320, 121.973305)
(9.089629, 0.671413)
(18.335535, 77.941714)
(10.185403, 0.697066)
};


==> figures/rawfiles/andersonvscond/andersonvscond_oampW_5.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(26.244871, 13.215363)
(17.552568, 17.575102)
(18.638512, 17.458363)
(18.546717, 11.872176)
(13.428638, 2.400898)
(16.794140, 36.383400)
(14.297143, 0.996715)
(17.171722, 19.819400)
(20.059292, 69.905633)
(11.256145, 1.473039)
(25.958267, 56.148753)
(14.636854, 14.432358)
(16.587755, 2.997509)
(8.500388, 1.218901)
(19.118383, 35.384059)
(19.355614, 86.111247)
(16.919485, 6.982495)
(10.740816, 0.919286)
(24.433674, 42.915278)
(15.328254, 5.885575)
(15.667542, 14.325202)
(32.651962, 136.114845)
(14.833853, 5.929440)
(24.772644, 29.596865)
(19.206205, 55.090332)
(18.807907, 57.554345)
(20.472019, 20.223850)
(24.486319, 78.227207)
(13.134361, 4.123993)
(14.394195, 1.761163)
(16.070848, 7.822428)
(25.167027, 46.812477)
(15.581610, 7.428723)
(17.096106, 15.785281)
(21.280998, 33.711246)
(23.876585, 45.308438)
(13.036207, 5.663250)
(22.731215, 65.189747)
(35.325077, 128.599324)
(24.573538, 27.980417)
(22.238827, 127.344119)
(17.241997, 38.357269)
(21.504358, 28.653758)
(16.334728, 18.709306)
(18.660828, 31.584973)
(10.326597, 0.479474)
(16.468248, 14.448580)
(13.946894, 6.961119)
(33.479321, 115.533678)
(13.391328, 8.614831)
(16.313137, 16.859823)
(17.417023, 25.684424)
(14.955702, 25.914733)
(23.593338, 40.456769)
(25.343109, 132.633033)
(28.576508, 105.730112)
(26.743855, 105.457015)
(17.670483, 9.764345)
(14.859500, 34.487936)
(13.146446, 15.457534)
(16.851610, 11.730871)
(24.674076, 80.917926)
(14.513160, 14.110297)
(18.443485, 17.230545)
(13.139583, 2.973897)
(13.289401, 1.852945)
(13.496741, 2.037040)
(17.107384, 3.074789)
(9.916093, 0.635562)
(12.541000, 3.786652)
(13.952982, 6.857228)
(19.874964, 83.943861)
(36.316109, 141.187532)
(14.172893, 3.632254)
(8.225883, 0.589236)
(13.984437, 19.779131)
(32.250385, 80.605731)
(20.073103, 15.670521)
(18.860682, 47.398704)
(21.450701, 35.458627)
(12.890105, 6.105768)
(20.801798, 33.666168)
(20.644512, 27.061260)
(19.323544, 47.555410)
(12.121391, 15.126105)
(15.076665, 5.212036)
(15.545311, 23.758901)
(15.126464, 58.592920)
(8.966540, 0.843358)
(14.076862, 19.491054)
(18.888176, 103.847809)
(12.218390, 4.765445)
(27.091944, 54.779785)
(8.184272, 0.598134)
(21.078032, 18.789568)
(34.766178, 134.277204)
(24.455320, 95.405653)
(9.089629, 0.623265)
(18.335535, 57.989808)
(10.185403, 0.703056)
};


==> figures/rawfiles/andersonvscond/andersonvscond_oampW_6.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(26.244871, 12.022041)
(17.552568, 18.159581)
(18.638512, 21.174660)
(18.546717, 15.498219)
(13.428638, 2.121334)
(16.794140, 111.025980)
(14.297143, 0.951886)
(17.171722, 23.635525)
(20.059292, 78.223182)
(11.256145, 1.269704)
(25.958267, 69.217283)
(14.636854, 11.651865)
(16.587755, 2.544879)
(8.500388, 1.288926)
(19.118383, 53.640187)
(19.355614, 94.132624)
(16.919485, 4.743346)
(10.740816, 0.936954)
(24.433674, 50.548323)
(15.328254, 7.044672)
(15.667542, 14.375657)
(32.651962, 134.141142)
(14.833853, 9.339874)
(24.772644, 32.891090)
(19.206205, 50.037343)
(18.807907, 72.155943)
(20.472019, 15.958277)
(24.486319, 85.245414)
(13.134361, 4.080515)
(14.394195, 1.348121)
(16.070848, 7.775311)
(25.167027, 54.513302)
(15.581610, 6.514093)
(17.096106, 27.761615)
(21.280998, 34.976190)
(23.876585, 61.380641)
(13.036207, 7.161789)
(22.731215, 106.981729)
(35.325077, 163.071021)
(24.573538, 48.462771)
(22.238827, 337.175226)
(17.241997, 51.408377)
(21.504358, 26.183837)
(16.334728, 45.214125)
(18.660828, 27.735091)
(10.326597, 0.478593)
(16.468248, 25.755342)
(13.946894, 6.966352)
(33.479321, 132.293923)
(13.391328, 9.316603)
(16.313137, 14.303753)
(17.417023, 22.787798)
(14.955702, 48.534876)
(23.593338, 50.308554)
(25.343109, 125.980862)
(28.576508, 146.703406)
(26.743855, 92.911181)
(17.670483, 7.139128)
(14.859500, 75.227747)
(13.146446, 9.925546)
(16.851610, 16.882046)
(24.674076, 105.651728)
(14.513160, 15.350930)
(18.443485, 26.629898)
(13.139583, 5.186246)
(13.289401, 1.882365)
(13.496741, 1.482392)
(17.107384, 3.434546)
(9.916093, 0.700765)
(12.541000, 4.071166)
(13.952982, 6.605585)
(19.874964, 92.705194)
(36.316109, 158.526447)
(14.172893, 13.454412)
(8.225883, 0.589270)
(13.984437, 19.808070)
(32.250385, 86.552984)
(20.073103, 20.957016)
(18.860682, 48.949958)
(21.450701, 33.073926)
(12.890105, 6.212676)
(20.801798, 95.528787)
(20.644512, 32.239850)
(19.323544, 42.527520)
(12.121391, 21.600565)
(15.076665, 4.671265)
(15.545311, 39.287092)
(15.126464, 84.352369)
(8.966540, 0.772826)
(14.076862, 23.977770)
(18.888176, 117.176875)
(12.218390, 4.305419)
(27.091944, 78.391509)
(8.184272, 0.674774)
(21.078032, 17.476503)
(34.766178, 154.570268)
(24.455320, 90.935560)
(9.089629, 0.630520)
(18.335535, 62.157182)
(10.185403, 0.610752)
};


==> figures/rawfiles/andersonvscond/andersonvscond_oampW_7.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(26.244871, 10.474139)
(17.552568, 19.118116)
(18.638512, 34.104504)
(18.546717, 25.594617)
(13.428638, 4.111515)
(16.794140, 91.875759)
(14.297143, 0.977486)
(17.171722, 21.549625)
(20.059292, 116.753591)
(11.256145, 1.265971)
(25.958267, 63.096954)
(14.636854, 13.051430)
(16.587755, 3.235073)
(8.500388, 1.428625)
(19.118383, 49.731112)
(19.355614, 308.518508)
(16.919485, 5.453142)
(10.740816, 1.208140)
(24.433674, 48.690800)
(15.328254, 12.908847)
(15.667542, 21.755417)
(32.651962, 143.209520)
(14.833853, 10.574450)
(24.772644, 55.414624)
(19.206205, 44.715291)
(18.807907, 107.626686)
(20.472019, 38.137033)
(24.486319, 103.050076)
(13.134361, 3.286935)
(14.394195, 1.637060)
(16.070848, 28.993592)
(25.167027, 67.592218)
(15.581610, 6.270230)
(17.096106, 37.968939)
(21.280998, 45.023327)
(23.876585, 53.372911)
(13.036207, 6.948125)
(22.731215, 73.309136)
(35.325077, 165.979609)
(24.573538, 27.788689)
(22.238827, 123.250525)
(17.241997, 53.228841)
(21.504358, 40.004948)
(16.334728, 36.701294)
(18.660828, 19.292306)
(10.326597, 0.480974)
(16.468248, 26.200106)
(13.946894, 6.953362)
(33.479321, 137.140347)
(13.391328, 37.359814)
(16.313137, 57.519274)
(17.417023, 22.521206)
(14.955702, 61.128916)
(23.593338, 57.119168)
(25.343109, 128.367358)
(28.576508, 96.263427)
(26.743855, 123.875664)
(17.670483, 3.732898)
(14.859500, 53.504990)
(13.146446, 24.092753)
(16.851610, 14.860221)
(24.674076, 107.117532)
(14.513160, 16.852006)
(18.443485, 24.998732)
(13.139583, 4.206025)
(13.289401, 2.467373)
(13.496741, 1.241503)
(17.107384, 2.061821)
(9.916093, 0.644872)
(12.541000, 4.221141)
(13.952982, 9.528282)
(19.874964, 131.915934)
(36.316109, 179.643143)
(14.172893, 6.778494)
(8.225883, 0.588938)
(13.984437, 31.740056)
(32.250385, 167.576323)
(20.073103, 24.045885)
(18.860682, 114.123919)
(21.450701, 100.338949)
(12.890105, 5.795560)
(20.801798, 76.510240)
(20.644512, 39.359856)
(19.323544, 74.166117)
(12.121391, 24.328726)
(15.076665, 5.542624)
(15.545311, 29.052684)
(15.126464, 196.601932)
(8.966540, 1.276892)
(14.076862, 39.150975)
(18.888176, 156.875422)
(12.218390, 4.818119)
(27.091944, 82.328433)
(8.184272, 0.671559)
(21.078032, 27.779693)
(34.766178, 143.123317)
(24.455320, 102.088169)
(9.089629, 0.634041)
(18.335535, 85.391143)
(10.185403, 0.743768)
};


==> figures/rawfiles/andersonvscond/andersonvscond_oampW_8.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(26.244871, 19.780089)
(17.552568, 19.189300)
(18.638512, 41.312835)
(18.546717, 20.502081)
(13.428638, 1.715901)
(16.794140, 50.622561)
(14.297143, 0.942075)
(17.171722, 22.662701)
(20.059292, 149.205589)
(11.256145, 1.266540)
(25.958267, 181.655340)
(14.636854, 19.720954)
(16.587755, 2.548574)
(8.500388, 1.284590)
(19.118383, 35.786978)
(19.355614, 178.854502)
(16.919485, 8.740932)
(10.740816, 0.939417)
(24.433674, 110.707769)
(15.328254, 23.745001)
(15.667542, 14.017693)
(32.651962, 333.961156)
(14.833853, 6.190909)
(24.772644, 39.107000)
(19.206205, 126.164924)
(18.807907, 74.540928)
(20.472019, 23.410613)
(24.486319, 212.184042)
(13.134361, 2.118417)
(14.394195, 1.516096)
(16.070848, 19.180165)
(25.167027, 83.621824)
(15.581610, 14.193454)
(17.096106, 18.951228)
(21.280998, 81.431803)
(23.876585, 75.139199)
(13.036207, 5.765602)
(22.731215, 160.746902)
(35.325077, 353.507636)
(24.573538, 57.743034)
(22.238827, 394.832533)
(17.241997, 61.849893)
(21.504358, 63.605586)
(16.334728, 75.182305)
(18.660828, 71.085666)
(10.326597, 0.480551)
(16.468248, 12.390327)
(13.946894, 6.555991)
(33.479321, 299.292810)
(13.391328, 13.771327)
(16.313137, 32.967254)
(17.417023, 28.839767)
(14.955702, 20.316610)
(23.593338, 80.218362)
(25.343109, 294.018102)
(28.576508, 280.492287)
(26.743855, 222.861263)
(17.670483, 8.050744)
(14.859500, 41.108444)
(13.146446, 21.156020)
(16.851610, 23.166089)
(24.674076, 201.642670)
(14.513160, 18.560462)
(18.443485, 37.692767)
(13.139583, 3.408605)
(13.289401, 2.442590)
(13.496741, 1.221127)
(17.107384, 3.969129)
(9.916093, 0.644828)
(12.541000, 4.051943)
(13.952982, 7.665076)
(19.874964, 263.426738)
(36.316109, 254.537553)
(14.172893, 7.460588)
(8.225883, 0.651002)
(13.984437, 18.445620)
(32.250385, 113.623360)
(20.073103, 19.491938)
(18.860682, 81.394639)
(21.450701, 40.379115)
(12.890105, 11.016249)
(20.801798, 48.583999)
(20.644512, 52.841956)
(19.323544, 69.993225)
(12.121391, 14.753771)
(15.076665, 9.902606)
(15.545311, 25.300735)
(15.126464, 96.230036)
(8.966540, 0.800886)
(14.076862, 93.627102)
(18.888176, 161.718465)
(12.218390, 4.703865)
(27.091944, 141.517990)
(8.184272, 0.710387)
(21.078032, 14.469580)
(34.766178, 303.745022)
(24.455320, 229.466654)
(9.089629, 0.624488)
(18.335535, 118.259006)
(10.185403, 0.609957)
};


==> figures/rawfiles/andersonvscond/andersonvscond_oampW_9.tex <==
\addplot+ [mark=none, ultra thick] coordinates{ 
(26.244871, 13.263103)
(17.552568, 17.315676)
(18.638512, 26.171088)
(18.546717, 13.322415)
(13.428638, 1.497944)
(16.794140, 25.943652)
(14.297143, 0.693264)
(17.171722, 16.408647)
(20.059292, 75.170307)
(11.256145, 1.266530)
(25.958267, 70.634929)
(14.636854, 11.823602)
(16.587755, 2.040131)
(8.500388, 1.090178)
(19.118383, 30.551771)
(19.355614, 89.263839)
(16.919485, 3.978523)
(10.740816, 0.935995)
(24.433674, 53.586688)
(15.328254, 10.133978)
(15.667542, 8.851507)
(32.651962, 156.919644)
(14.833853, 4.211444)
(24.772644, 29.875079)
(19.206205, 47.394965)
(18.807907, 36.213257)
(20.472019, 16.067602)
(24.486319, 88.096984)
(13.134361, 1.530151)
(14.394195, 1.309242)
(16.070848, 7.146768)
(25.167027, 39.998265)
(15.581610, 6.178185)
(17.096106, 11.854502)
(21.280998, 49.621940)
(23.876585, 37.352775)
(13.036207, 4.365404)
(22.731215, 76.018475)
(35.325077, 180.593707)
(24.573538, 28.686773)
(22.238827, 141.289094)
(17.241997, 44.568821)
(21.504358, 34.252126)
(16.334728, 17.887149)
(18.660828, 26.455987)
(10.326597, 0.496515)
(16.468248, 6.978323)
(13.946894, 6.930422)
(33.479321, 141.815987)
(13.391328, 6.507811)
(16.313137, 18.119141)
(17.417023, 22.679446)
(14.955702, 7.970242)
(23.593338, 41.566021)
(25.343109, 135.136946)
(28.576508, 110.133276)
(26.743855, 145.909823)
(17.670483, 5.446619)
(14.859500, 32.375321)
(13.146446, 17.070232)
(16.851610, 9.341698)
(24.674076, 110.519655)
(14.513160, 9.300717)
(18.443485, 14.083366)
(13.139583, 2.077613)
(13.289401, 1.727095)
(13.496741, 2.101948)
(17.107384, 1.967357)
(9.916093, 0.605884)
(12.541000, 3.928758)
(13.952982, 5.806000)
(19.874964, 93.510916)
(36.316109, 196.890791)
(14.172893, 4.071675)
(8.225883, 0.589395)
(13.984437, 11.510112)
(32.250385, 72.032893)
(20.073103, 13.364444)
(18.860682, 36.598866)
(21.450701, 28.937418)
(12.890105, 5.308068)
(20.801798, 27.053698)
(20.644512, 38.654319)
(19.323544, 58.151150)
(12.121391, 11.817965)
(15.076665, 4.239731)
(15.545311, 16.945514)
(15.126464, 38.303217)
(8.966540, 0.675387)
(14.076862, 24.999688)
(18.888176, 104.567977)
(12.218390, 4.082551)
(27.091944, 71.242249)
(8.184272, 0.585501)
(21.078032, 10.420242)
(34.766178, 148.033646)
(24.455320, 92.506757)
(9.089629, 0.639939)
(18.335535, 75.895463)
(10.185403, 0.597366)
};


==> noncorrelated.tex <==
\section{From \gls{iid} Gaussian Channels to the Real~World}\label{ch:iid}
In this section, we first compare the performance of different schemes on \gls{iid} Gaussian $\textbf{H}_{ij}\sim \mathcal{CN}(0,\frac{1}{N_r})$ channels. We then evaluate the assumption of Gaussian iid channels. Results show that adding a very few degrees of freedom to the one of classic iterative algorithms, \gls{amp}, can perform better than or equal to the state-of-the-art schemes on these \gls{iid} Gaussian channels. 
\subsection{MIMO Schemes Performance Benchmark}
\begin{figure}[!ht]
    \centering
    \input{figures/iid_combined.tex}
    \caption{SER vs. SNR comparison of different MIMO detection schemes for QAM modulations on iid Complex-Guassian $64\times32$ channels.}
    \label{fig:iid}
\end{figure}
\Cref{fig:iid} compares the performance of the  state-of-the-art MIMO schemes on $64\times32$ Complex-Gaussian \gls{iid} channels. The \glsfirst{ml} curve stands for the optimal accuracy. There is more than one scheme which performs close to the optimal for each modulation. The set of near-optimal schemes shrinks while we move toward higher modulations. 
We also add a simple baseline here which comes from a little tweak to the \gls{amp} algorithm.
\begin{align}\label{eq:our_design}
\begin{split}
    \textbf{z}_t &= \xh_{t} + \theta_t^{(1)}\Hb^T (\y - \Hb\xh_t)\\
    \xh_{t+1} &=\theta_t^{(2)}\eta^g_t\left( \textbf{z}_t;\sigma_t^2 \right) + \theta_t^{(3)} \textbf{z}_t
\end{split}
\end{align}
\Gls{amp} follows a very similar structure except with $\theta_t^{(1)}=1$. We have also removed the Onsager term in the first update equation. Second update equation is disccussed further in details in \Cref{sec:ourdesign}. Parameters $\theta_t^{(1:3)}$ are trainable scalars. This scheme is labeled as \emph{baseline} in \Cref{fig:iid} and much less complexity than the two other learning based schemes \detnet and OAMPNet. We see that adding just a few degrees of freedom to the current scheme \gls{amp} can give us better or equal performance relative to huge deep learning models like \detnet and outperform classics like \gls{sdr}.

\subsection{Do we really have multiple choices for MIMO detection?}
\begin{figure}
    \centering
    \input{figures/H00.tex}
    \caption{SER vs. SNR for a sample realization of $64\times 16$ correlated channel for state-of-the-art schemes on uncorrelated channels. \sys shows promising performance in case of correlated channels.}
    \label{fig:H00}
\end{figure}
Although we have multiple near-optimal choices for \gls{iid} Gaussian channels, they all perform poorly on real channel scenarios. \Cref{fig:H00} shows the performance of OAMPNet on a real channel scenario with correlations being present. We see an astonishing $\approx$11dB performance difference between MMSE and \gls{ml} at SER of 0.01. This deviation can be huge compared with 2-3dB difference we have for iid channels in \Cref{fig:iid}. DetNet is not shown here as it is not possible to train it to a reasonable performance on these channel samples and it has stability issues during the training. \Gls{amp} performs infamously poor on correlated channels. We also do not consider any approach more complex than \detnet here because of their complexity. Thus, \gls{sdr} algorithms are not among our tests.
We propose an iterative approach called \sys which closes the 11dB gap with the optimal toward 2dB. Before that, we first study what goes wrong with current state-of-the-art iterative schemes \gls{amp}, OAMPNet, and \detnet in the case of more realistic channels. 

